Design Aspects of Multi-Soliton Pulses for Optical Fiber Transmission

We explain how to optimize the nonlinear spectrum of multi-soliton pulses by considering the practical constraints of transmitter, receiver, and lumped-amplified link. The optimization is applied for the experimental transmission of 2ns soliton pulses with independent on-off keying of 10 eigenvalues over 2000 km of NZ-DSF fiber spans.

==> sym19_bandwidth.tex <==
% This file was created by matlab2tikz.
%%
%%The latest updates can be retrieved from
%%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%%where you can also make suggestions and rate matlab2tikz.
%%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%%
%\begin{tikzpicture}

\begin{axis}[%
width=0.951\picwidth,
height=\picheight,
at={(0\picwidth,0\picheight)},
scale only axis,
xmin=0,
xmax=2032,
xtick={0,500,1000,1500,2000},
xticklabels={{0},{.5},{1.0},{1.5},{2.0}},
xlabel={fiber length z, ($\times$1000 km)},
ymin=7,
ymax=15,
ytick={ 7,  9, 11, 13, 15},
ylabel={Bandwidth (GHz)},
axis background/.style={fill=white}
]
\addplot [color=mycolor1,solid,line width=2.0pt,forget plot]
  table[row sep=crcr]{%
0	8\\
24.2	8\\
48.4	8\\
72.6	8.5\\
96.8	8.5\\
121	8.5\\
145.2	9\\
169.4	9\\
193.6	9.5\\
217.8	10\\
242	10\\
266.2	11\\
290.4	12\\
314.6	12.5\\
338.8	13\\
363	13.5\\
387.2	13.5\\
411.4	14\\
435.6	14\\
459.8	13.5\\
484	13.5\\
508.2	13\\
532.4	12.5\\
556.6	12\\
580.8	11.5\\
605	11.5\\
629.2	11\\
653.4	11\\
677.6	11\\
701.8	11.5\\
726	11.5\\
750.2	12\\
774.4	12.5\\
798.6	12.5\\
822.8	13\\
847	13\\
871.2	13.5\\
895.4	13.5\\
919.6	13\\
943.8	13\\
968	12.5\\
992.2	12.5\\
1016.4	11.5\\
1040.6	10.5\\
1064.8	10\\
1089	10\\
1113.2	10\\
1137.4	10\\
1161.6	10\\
1185.8	10\\
1210	10\\
1234.2	10\\
1258.4	9.5\\
1282.6	9.5\\
1306.8	9.5\\
1331	9.5\\
1355.2	9.5\\
1379.4	9.5\\
1403.6	9.5\\
1427.8	10\\
1452	12\\
1476.2	13\\
1500.4	13.5\\
1524.6	13.5\\
1548.8	14\\
1573	14\\
1597.2	14\\
1621.4	13.5\\
1645.6	13.5\\
1669.8	13.5\\
1694	13\\
1718.2	12.5\\
1742.4	12\\
1766.6	11.5\\
1790.8	11\\
1815	10.5\\
1839.2	10\\
1863.4	9.5\\
1887.6	9.5\\
1911.8	9.5\\
1936	9.5\\
1960.2	9\\
1984.4	9\\
2008.6	9\\
2032.8	9.5\\
};
\addplot [color=mycolor2,solid,line width=2.0pt,forget plot]
  table[row sep=crcr]{%
0	7.5\\
24.2	7.5\\
48.4	7.5\\
72.6	7.5\\
96.8	7.5\\
121	7.5\\
145.2	7.5\\
169.4	8\\
193.6	8\\
217.8	8.5\\
242	9\\
266.2	9.5\\
290.4	9.5\\
314.6	10\\
338.8	10.5\\
363	11\\
387.2	11.5\\
411.4	12\\
435.6	12\\
459.8	12\\
484	12\\
508.2	12\\
532.4	11.5\\
556.6	11\\
580.8	10.5\\
605	10.5\\
629.2	10.5\\
653.4	10.5\\
677.6	10.5\\
701.8	10.5\\
726	10.5\\
750.2	10.5\\
774.4	10.5\\
798.6	11\\
822.8	11\\
847	11\\
871.2	11\\
895.4	11\\
919.6	11\\
943.8	11\\
968	11\\
992.2	10.5\\
1016.4	10\\
1040.6	10\\
1064.8	9.5\\
1089	9.5\\
1113.2	9.5\\
1137.4	9.5\\
1161.6	9.5\\
1185.8	9.5\\
1210	10\\
1234.2	10\\
1258.4	10\\
1282.6	10\\
1306.8	10.5\\
1331	10.5\\
1355.2	11\\
1379.4	11.5\\
1403.6	12.5\\
1427.8	12.5\\
1452	12.5\\
1476.2	12.5\\
1500.4	12.5\\
1524.6	12.5\\
1548.8	12.5\\
1573	12.5\\
1597.2	12.5\\
1621.4	12.5\\
1645.6	12.5\\
1669.8	12.5\\
1694	12.5\\
1718.2	12\\
1742.4	11.5\\
1766.6	10.5\\
1790.8	10\\
1815	9\\
1839.2	9\\
1863.4	9\\
1887.6	8.5\\
1911.8	8.5\\
1936	8.5\\
1960.2	8.5\\
1984.4	8.5\\
2008.6	8.5\\
2032.8	8.5\\
};
\end{axis}

\begin{axis}[%
width=1.227\picwidth,
height=1.227\picheight,
at={(-0.16\picwidth,-0.135\picheight)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
hide axis,
axis x line*=bottom,
axis y line*=left
]
\node[below right, align=left, text=black]
at (rel axis cs:0.45,0.92) {B};
\node[below right, align=left, text=black]
at (rel axis cs:0.26,0.92) {A};
\node[below right, align=left, text=black]
at (rel axis cs:0.70,0.92) {C};
\node[below right, align=left, text=black]
at (rel axis cs:0.70,0.65) {D};
\end{axis}
%\end{tikzpicture}%

==> sym19_new_EV.tex <==
%% This file was created by matlab2tikz.
%%
%%The latest updates can be retrieved from
%%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%%where you can also make suggestions and rate matlab2tikz.
%%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
%\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
%\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%%
%\begin{tikzpicture}

\begin{axis}[%
width=0.951\picwidth,
height=.40\picheight,
at={(0\picwidth,0\picheight)},
scale only axis,
xmin=0,
xmax=2032,
xtick={0,500,1000,1500,2000},
xticklabels={{0},{.5},{1.0},{1.5},{2.0}},
%xlabel={\footnotesize fiber length z, ($\times$1000 km)},
ymin=0.8,
ymax=2.2,
ytick={0.8, 1.2, 1.6,   2},
ylabel={\footnotesize Imag($\lambda_i(z)$)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot [color=mycolor1,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	2.00039597784803\\
24.2	2.0015401312389\\
48.4	2.00121166997855\\
72.6	2.00087394185858\\
96.8	1.99998662608149\\
121	2.00013507648919\\
145.2	1.99964786740008\\
169.4	1.99921057638436\\
193.6	1.99860971395534\\
217.8	1.9979117637632\\
242	1.99772574199587\\
266.2	1.99759396202405\\
290.4	1.99744275631669\\
314.6	2.00039659120795\\
338.8	2.00219539356191\\
363	2.00466054731257\\
387.2	2.00768945313036\\
411.4	2.01100253073868\\
435.6	2.01415779800903\\
459.8	2.01667802950645\\
484	2.01821489947153\\
508.2	2.01865094210449\\
532.4	2.01810081988359\\
556.6	2.01683475343899\\
580.8	2.01517943294232\\
605	2.01343750183263\\
629.2	2.01183840868164\\
653.4	2.00800506126319\\
677.6	2.00756389118379\\
701.8	2.00640091904016\\
726	2.00644988799975\\
750.2	2.00519679136268\\
774.4	2.00477937686651\\
798.6	2.00461488008207\\
822.8	2.00394888928609\\
847	2.00493961045979\\
871.2	2.00461583764886\\
895.4	2.00478441581456\\
919.6	2.00443904130636\\
943.8	2.00439525747329\\
968	2.00466446920806\\
992.2	2.00516353713943\\
1016.4	2.00577662244889\\
1040.6	2.00637795739712\\
1064.8	2.00687598881752\\
1089	2.00723304465825\\
1113.2	2.00744734910263\\
1137.4	2.0059228196884\\
1161.6	2.00618728810514\\
1185.8	2.00684741366715\\
1210	2.00757017537419\\
1234.2	2.00708496132862\\
1258.4	2.0062534078164\\
1282.6	2.00598930129282\\
1306.8	2.00613664434122\\
1331	2.00617097889297\\
1355.2	2.00620391523913\\
1379.4	2.00356603556421\\
1403.6	2.00240639936354\\
1427.8	2.00115542369178\\
1452	1.99986164019942\\
1476.2	1.99855965064605\\
1500.4	1.99728785940336\\
1524.6	1.99614005713275\\
1548.8	1.99531335026854\\
1573	1.99509589916422\\
1597.2	1.99846932245681\\
1621.4	2.00347562422452\\
1645.6	1.99985826623081\\
1669.8	2.00265620125375\\
1694	2.00526978653707\\
1718.2	2.00727790187985\\
1742.4	2.0084872203557\\
1766.6	2.00892351672854\\
1790.8	2.00874557487671\\
1815	2.0081535403305\\
1839.2	2.00732703978796\\
1863.4	2.00640029829857\\
1887.6	2.00533088168739\\
1911.8	2.00461468279509\\
1936	2.00404783799123\\
1960.2	2.00301097749184\\
1984.4	2.00250634789193\\
2008.6	2.00156728142121\\
2032.8	2.00099325474235\\
};
\addplot [color=mycolor2,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.99995376618847\\
24.2	1.9994905649516\\
48.4	2.00160073545461\\
72.6	2.00074658422794\\
96.8	2.00150134801477\\
121	2.00178248017798\\
145.2	2.00292398622658\\
169.4	2.00325314431696\\
193.6	2.00379584835209\\
217.8	2.00460202922298\\
242	2.00474156579654\\
266.2	2.00486889879577\\
290.4	2.00802118343077\\
314.6	2.00454305330929\\
338.8	2.00347471534376\\
363	2.00243739244896\\
387.2	2.00087885283384\\
411.4	1.99802416490416\\
435.6	1.99466799880928\\
459.8	1.99387507491093\\
484	1.99089127907083\\
508.2	1.98877686834082\\
532.4	1.98769248352866\\
556.6	1.98758862254362\\
580.8	1.98826297381995\\
605	1.98943642512791\\
629.2	1.99081936823274\\
653.4	1.99215563372559\\
677.6	1.99324352176315\\
701.8	1.99254015767646\\
726	1.99252505213145\\
750.2	1.99161634267195\\
774.4	1.9916760381831\\
798.6	1.99108784742761\\
822.8	1.99043548978149\\
847	1.98898568096659\\
871.2	1.98779241278001\\
895.4	1.98712491406826\\
919.6	1.98718937539597\\
943.8	1.98805091207788\\
968	1.98961307659993\\
992.2	1.99162362827101\\
1016.4	1.99374839335292\\
1040.6	1.99565598685935\\
1064.8	1.99708409334577\\
1089	1.99787108457015\\
1113.2	1.99794788293545\\
1137.4	1.99731514309177\\
1161.6	1.99601679273227\\
1185.8	1.99412137515199\\
1210	1.99172670992377\\
1234.2	1.98898295302589\\
1258.4	1.9861225612309\\
1282.6	1.9834947430441\\
1306.8	1.98159914486365\\
1331	1.9810885336757\\
1355.2	1.98268065017121\\
1379.4	1.9869425254114\\
1403.6	1.99398947940369\\
1427.8	2.00323182936815\\
1452	2.01335437953663\\
1476.2	2.02266181075799\\
1500.4	2.0296518049425\\
1524.6	2.03340905937641\\
1548.8	2.03361793044845\\
1573	2.03041341711185\\
1597.2	2.02435445412542\\
1621.4	2.01648773940839\\
1645.6	2.0082473430818\\
1669.8	2.00361981291583\\
1694	1.99587475469817\\
1718.2	1.99133721242126\\
1742.4	1.99204809520782\\
1766.6	1.99242580265862\\
1790.8	1.99351863304661\\
1815	1.99485385888702\\
1839.2	1.99491878664065\\
1863.4	1.99571648957971\\
1887.6	1.99656969041729\\
1911.8	1.99733803096459\\
1936	1.99789890412563\\
1960.2	1.99854647686316\\
1984.4	1.99882359795819\\
2008.6	1.99906774640745\\
2032.8	1.99948691636717\\
};
\addplot [color=mycolor3,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.99969524029269\\
24.2	1.99860805552791\\
48.4	1.99993007401376\\
72.6	1.9996927615363\\
96.8	2.00063691897737\\
121	1.9997144558168\\
145.2	2.00050241371414\\
169.4	2.00084539123028\\
193.6	2.00150412760574\\
217.8	2.00211910867506\\
242	2.00247616354102\\
266.2	2.00333078488036\\
290.4	2.00357047014066\\
314.6	2.00361949023476\\
338.8	2.00341811959654\\
363	2.00290329333013\\
387.2	2.00202536892221\\
411.4	2.00082468597011\\
435.6	1.99947359654908\\
459.8	1.99822727346983\\
484	1.99733472619833\\
508.2	1.99697266798293\\
532.4	1.99721765940987\\
556.6	1.99805396831259\\
580.8	1.99940159908186\\
605	2.00114882012363\\
629.2	2.00317291039745\\
653.4	2.00535484634748\\
677.6	2.0075828217798\\
701.8	2.00974808571483\\
726	2.01173130939915\\
750.2	2.01338047895909\\
774.4	2.01451167877368\\
798.6	2.01491516917831\\
822.8	2.01436758973515\\
847	2.01268195370608\\
871.2	2.00978164163687\\
895.4	2.00579391253012\\
919.6	2.00108725440142\\
943.8	1.99622914209691\\
968	1.99185731345696\\
992.2	1.98849364089417\\
1016.4	1.98644735255095\\
1040.6	1.98578340386194\\
1064.8	1.98637377835435\\
1089	1.98802536188271\\
1113.2	1.9905546211172\\
1137.4	1.99298648676525\\
1161.6	1.99849510453055\\
1185.8	2.00259744944457\\
1210	2.00819551069979\\
1234.2	2.0146846880488\\
1258.4	2.02201026532587\\
1282.6	2.02990207159137\\
1306.8	2.03774386892517\\
1331	2.04446066205824\\
1355.2	2.04854714238395\\
1379.4	2.04841215882458\\
1403.6	2.04303570724015\\
1427.8	2.032628430914\\
1452	2.01881962999211\\
1476.2	2.00413967570171\\
1500.4	1.99104998960712\\
1524.6	1.98114994867576\\
1548.8	1.97498156310127\\
1573	1.97229408237692\\
1597.2	1.97240230100059\\
1621.4	1.97444760636583\\
1645.6	1.9775682071942\\
1669.8	1.9810367129809\\
1694	1.98435667356981\\
1718.2	1.98728313556241\\
1742.4	1.98976303824485\\
1766.6	1.99184682657886\\
1790.8	1.99361567478799\\
1815	1.99340239552271\\
1839.2	1.99367244361928\\
1863.4	1.99644199351446\\
1887.6	1.99601010928096\\
1911.8	1.9983582936563\\
1936	1.9997462371391\\
1960.2	2.00071051463226\\
1984.4	2.00118907419616\\
2008.6	2.00165457565933\\
2032.8	2.00239789688173\\
};
\addplot [color=mycolor4,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.9997372552601\\
24.2	2.0000731685299\\
48.4	2.00141953275979\\
72.6	2.00076324925706\\
96.8	2.00052425318664\\
121	2.00192826127513\\
145.2	2.00169425444777\\
169.4	2.00179689936048\\
193.6	2.00032450697547\\
217.8	2.00025007783514\\
242	1.99961364551607\\
266.2	1.99916480650968\\
290.4	1.99832676440458\\
314.6	1.99767626661379\\
338.8	1.99741413802977\\
363	1.99698062866926\\
387.2	1.99690024977068\\
411.4	1.99721767607308\\
435.6	1.99841720282872\\
459.8	2.00043389225067\\
484	2.00504642715806\\
508.2	2.00744670331189\\
532.4	2.00949973403411\\
556.6	2.0110259559637\\
580.8	2.01194122994987\\
605	2.0122373622548\\
629.2	2.0119553994612\\
653.4	2.01116072325157\\
677.6	2.00993255400114\\
701.8	2.00838842729757\\
726	2.00668958272357\\
750.2	2.00060512051506\\
774.4	1.99871240796623\\
798.6	1.9988054065798\\
822.8	2.00018299927742\\
847	2.00423735220217\\
871.2	2.00550217658005\\
895.4	2.00656242574423\\
919.6	2.00679205981388\\
943.8	2.00581437127772\\
968	2.00367393083981\\
992.2	2.00087153019894\\
1016.4	1.99813216337013\\
1040.6	1.99612118400933\\
1064.8	1.99527335113427\\
1089	1.99574567922513\\
1113.2	1.9930870694454\\
1137.4	1.99684238402436\\
1161.6	2.0019821681731\\
1185.8	2.00802328755411\\
1210	2.01229415386525\\
1234.2	2.01625745632066\\
1258.4	2.01935314728609\\
1282.6	2.02093857431197\\
1306.8	2.02036847941072\\
1331	2.01716516900434\\
1355.2	2.01127214918124\\
1379.4	2.00325392768608\\
1403.6	1.9942708862435\\
1427.8	1.98582489260114\\
1452	1.97941618057317\\
1476.2	1.97618027634907\\
1500.4	1.97653531123411\\
1524.6	1.97997525794785\\
1548.8	1.98516947001566\\
1573	1.99037601148185\\
1597.2	1.99401337525689\\
1621.4	1.99519527936759\\
1645.6	1.99402906248629\\
1669.8	1.99150290121205\\
1694	1.98896807992916\\
1718.2	1.98750400953201\\
1742.4	1.98754960093255\\
1766.6	1.98894544066195\\
1790.8	1.99122013614665\\
1815	1.99386940619621\\
1839.2	1.99670646628115\\
1863.4	1.99894707086911\\
1887.6	2.00143274105703\\
1911.8	2.00232379397747\\
1936	2.00318962408675\\
1960.2	2.00467148625505\\
1984.4	2.00504333381908\\
2008.6	2.00593644537794\\
2032.8	2.00577215970319\\
};
\addplot [color=mycolor5,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	2.00008305198325\\
24.2	2.00005298413283\\
48.4	2.00083795077248\\
72.6	2.00053641892495\\
96.8	2.00022618174214\\
121	2.00022406012699\\
145.2	2.00106430296212\\
169.4	2.00132802480266\\
193.6	2.00151337745705\\
217.8	2.00175059265342\\
242	2.00207327131712\\
266.2	2.00268907736323\\
290.4	2.00302665494802\\
314.6	2.00376255869614\\
338.8	2.00445197552449\\
363	2.00511939649247\\
387.2	2.00569534911695\\
411.4	2.00608137843615\\
435.6	2.00578997476074\\
459.8	2.00472498205644\\
484	2.00321225475028\\
508.2	2.00131551980065\\
532.4	1.99991188463066\\
556.6	1.99882320684535\\
580.8	1.99837446535271\\
605	1.99764390899778\\
629.2	1.99752707514519\\
653.4	1.99658427041119\\
677.6	1.9964304213656\\
701.8	1.99592642634486\\
726	1.99515856860296\\
750.2	1.99498337265173\\
774.4	1.99464941011587\\
798.6	1.99403314297115\\
822.8	1.99274917095369\\
847	1.99095814928547\\
871.2	1.99446541368297\\
895.4	1.9947748927275\\
919.6	1.99581260223147\\
943.8	1.99757830510234\\
968	1.99984396342075\\
992.2	2.00221430752104\\
1016.4	1.9967509046739\\
1040.6	2.00126145511595\\
1064.8	2.00436432992639\\
1089	2.00582864924041\\
1113.2	2.00491928630537\\
1137.4	2.00211172202832\\
1161.6	1.99906427986764\\
1185.8	1.99447021269117\\
1210	1.99136173570687\\
1234.2	1.99064646982885\\
1258.4	1.9874313575961\\
1282.6	1.98475052114621\\
1306.8	1.98308223678246\\
1331	1.9829530224959\\
1355.2	1.98482599026842\\
1379.4	1.98892560384465\\
1403.6	1.99506196267418\\
1427.8	2.00255050968255\\
1452	2.01031611968392\\
1476.2	2.01717891781299\\
1500.4	2.0222043567765\\
1524.6	2.02493727368282\\
1548.8	2.02541230835353\\
1573	2.023992777798\\
1597.2	2.02117902944756\\
1621.4	2.01748385416057\\
1645.6	2.01339239436484\\
1669.8	2.00935463282732\\
1694	2.00575770685912\\
1718.2	2.00286364827309\\
1742.4	1.9998717076056\\
1766.6	1.99770494538988\\
1790.8	1.99657373998441\\
1815	1.99622440959405\\
1839.2	1.99647717593024\\
1863.4	1.99619883451567\\
1887.6	1.99609171600741\\
1911.8	1.99695246560358\\
1936	1.99796565442471\\
1960.2	1.99859946871284\\
1984.4	1.99911111552419\\
2008.6	1.99953301204974\\
2032.8	1.99949739024823\\
};
\addplot [color=mycolor6,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.00140200454495\\
24.2	1.00003735271358\\
48.4	1.0010097410524\\
72.6	0.999504010170033\\
96.8	0.998892413565417\\
121	0.998696406061256\\
145.2	0.998043434769958\\
169.4	0.996914728430984\\
193.6	0.996123172506774\\
217.8	0.995410724065416\\
242	0.994027553736889\\
266.2	0.992669290626826\\
290.4	0.991656522856861\\
314.6	0.990564213379333\\
338.8	0.987619048722421\\
363	0.98665830944376\\
387.2	0.986050224477265\\
411.4	0.985913855703507\\
435.6	0.986294776988874\\
459.8	0.98712895710477\\
484	0.988248843774164\\
508.2	0.98943118859167\\
532.4	0.990463284817154\\
556.6	0.991198124648918\\
580.8	0.991583031661786\\
605	0.991657385712934\\
629.2	0.991532862638283\\
653.4	0.991366490029855\\
677.6	0.991339007835171\\
701.8	0.991614237899717\\
726	0.992327021552983\\
750.2	0.993556165879914\\
774.4	0.99628621976458\\
798.6	0.997797397819517\\
822.8	1.00000896027029\\
847	1.0021789197574\\
871.2	1.00481501904614\\
895.4	1.00795844918694\\
919.6	1.01061860038788\\
943.8	1.01209239978895\\
968	1.01273112668607\\
992.2	1.01250522250656\\
1016.4	1.0115089629617\\
1040.6	1.00992676791062\\
1064.8	1.0079892020694\\
1089	1.00787214310514\\
1113.2	1.00504724479618\\
1137.4	1.00214072939274\\
1161.6	1.00027139021667\\
1185.8	0.99835871977784\\
1210	0.996472580725726\\
1234.2	0.995850618960615\\
1258.4	0.995156698798144\\
1282.6	0.994069984716626\\
1306.8	0.992648084070601\\
1331	0.992213212331382\\
1355.2	0.991947251678231\\
1379.4	0.991133426917804\\
1403.6	0.987372073396704\\
1427.8	0.98757934788\\
1452	0.988220691710769\\
1476.2	0.989180920339001\\
1500.4	0.990348628049672\\
1524.6	0.991681644284055\\
1548.8	0.993220710504444\\
1573	0.995028278988132\\
1597.2	0.997081377039897\\
1621.4	0.9991918558132\\
1645.6	1.00568285922615\\
1669.8	1.00706975231942\\
1694	1.00730823441215\\
1718.2	1.00255435613032\\
1742.4	1.00182156530511\\
1766.6	1.00312420205638\\
1790.8	1.00147780680073\\
1815	1.0001153901045\\
1839.2	1.00033083282113\\
1863.4	1.00002548217767\\
1887.6	0.999698323547551\\
1911.8	0.998745775007463\\
1936	0.998492727808794\\
1960.2	0.998107620375196\\
1984.4	0.998422373479226\\
2008.6	0.998772632753738\\
2032.8	0.999604681780786\\
};
\addplot [color=mycolor7,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	0.999738601336091\\
24.2	0.999061579274827\\
48.4	1.00072163456722\\
72.6	1.00157680535079\\
96.8	1.00297007363451\\
121	1.0027199327951\\
145.2	1.00476155308907\\
169.4	1.00561874411126\\
193.6	1.00717437060678\\
217.8	1.0080940629584\\
242	1.00876425423469\\
266.2	1.01078465517397\\
290.4	1.01150327789347\\
314.6	1.01187146427476\\
338.8	1.01179629349543\\
363	1.01121438402773\\
387.2	1.01011884030935\\
411.4	1.00857823904303\\
435.6	1.0067333470242\\
459.8	1.00477361949674\\
484	1.00289579698897\\
508.2	1.0012531852298\\
532.4	0.999509877627236\\
556.6	0.999777876419414\\
580.8	0.999421543478081\\
605	0.999970164181031\\
629.2	0.997938513673134\\
653.4	0.996508331070997\\
677.6	0.99567200965448\\
701.8	0.995522524890333\\
726	0.995053237808864\\
750.2	0.995261189368608\\
774.4	0.995408862844733\\
798.6	0.996901211091557\\
822.8	0.997608191928894\\
847	0.998976660918622\\
871.2	1.00061928344941\\
895.4	1.00229163103969\\
919.6	1.00373022837334\\
943.8	0.999398680200687\\
968	0.998668098849031\\
992.2	0.998222619741988\\
1016.4	0.997774949972846\\
1040.6	0.998242305376668\\
1064.8	1.00135933963167\\
1089	1.0001220041178\\
1113.2	0.99896276963666\\
1137.4	0.99783981688898\\
1161.6	0.996650873740862\\
1185.8	0.993205830538332\\
1210	0.991562686555252\\
1234.2	0.991487525129381\\
1258.4	0.988997442359275\\
1282.6	0.986199176170191\\
1306.8	0.983328496584263\\
1331	0.980784668135364\\
1355.2	0.979103839761014\\
1379.4	0.978851423502406\\
1403.6	0.980445950744362\\
1427.8	0.983975045628742\\
1452	0.989089375960182\\
1476.2	0.995063941853951\\
1500.4	1.00106654948808\\
1524.6	1.00651686327615\\
1548.8	1.01128328059308\\
1573	1.01556946536641\\
1597.2	1.01958589801191\\
1621.4	1.02324555223125\\
1645.6	1.02609364006515\\
1669.8	1.02752559972386\\
1694	1.02714874120094\\
1718.2	1.02502618104376\\
1742.4	1.0216413542778\\
1766.6	1.01765227365181\\
1790.8	1.01363893606135\\
1815	1.00997836692382\\
1839.2	1.00807249537206\\
1863.4	1.00457596228436\\
1887.6	1.00333174330601\\
1911.8	1.00089821710631\\
1936	1.00060479793291\\
1960.2	0.99896942406494\\
1984.4	0.998682588894227\\
2008.6	0.99675332049737\\
2032.8	0.99498486761761\\
};
\addplot [color=mycolor1,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	0.999012857983662\\
24.2	0.998344973329982\\
48.4	0.998392966012247\\
72.6	0.997002843393349\\
96.8	0.996165876374637\\
121	0.995027760942464\\
145.2	0.994140520994415\\
169.4	0.994425249567027\\
193.6	0.993522191632717\\
217.8	0.992708114127574\\
242	0.992032344189933\\
266.2	0.991554384326307\\
290.4	0.991339713211834\\
314.6	0.991457489851007\\
338.8	0.991970375772132\\
363	0.992904681400331\\
387.2	0.994225454675264\\
411.4	1.00128610640688\\
435.6	1.0033863427512\\
459.8	1.00468685400618\\
484	1.00454020777926\\
508.2	1.00275290321541\\
532.4	1.00073427502602\\
556.6	0.999326306530733\\
580.8	0.99861465137744\\
605	0.997308663293391\\
629.2	0.998476752896569\\
653.4	0.998152161642196\\
677.6	0.999581418326023\\
701.8	1.00011227418342\\
726	1.00066684017809\\
750.2	1.00119685424751\\
774.4	1.00127100361888\\
798.6	1.00040493242143\\
822.8	0.999345821927487\\
847	0.997744939376904\\
871.2	0.99603741567223\\
895.4	0.994649765311803\\
919.6	0.994312920432533\\
943.8	0.994647987683815\\
968	0.996263974687451\\
992.2	0.99848876294486\\
1016.4	1.00091883992439\\
1040.6	1.0034708516592\\
1064.8	1.00509672379181\\
1089	1.00596114756741\\
1113.2	1.00567937481306\\
1137.4	1.00459319860965\\
1161.6	1.00316473840933\\
1185.8	1.00123933844192\\
1210	1.00058820623984\\
1234.2	1.00039300906114\\
1258.4	1.00177998088093\\
1282.6	1.00241218721374\\
1306.8	1.00390012635467\\
1331	1.00543301226869\\
1355.2	1.00768125081297\\
1379.4	1.00976342165442\\
1403.6	1.01104853778794\\
1427.8	1.01091854188936\\
1452	1.00898750805135\\
1476.2	1.0067481762445\\
1500.4	1.00027612744033\\
1524.6	0.994777303214559\\
1548.8	0.989728979908245\\
1573	0.986042457126457\\
1597.2	0.984438698649508\\
1621.4	0.985263732266072\\
1645.6	0.988319759224482\\
1669.8	0.992847020892332\\
1694	0.997757398150289\\
1718.2	1.00203423497052\\
1742.4	1.00506603250733\\
1766.6	1.00672903435211\\
1790.8	1.0075444074063\\
1815	1.00683460339579\\
1839.2	1.00436654667648\\
1863.4	1.00382598082579\\
1887.6	1.00178422387405\\
1911.8	1.0017651275783\\
1936	1.00078453523658\\
1960.2	0.999692163084557\\
1984.4	0.998277554224677\\
2008.6	0.997737569145298\\
2032.8	0.996909179536882\\
};
\end{axis}

\begin{axis}[%
width=1.227\picwidth,
height=1.227\picheight,
at={(-0.16\picwidth,-0.135\picheight)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
hide axis,
axis x line*=bottom,
axis y line*=left
]
\node[below right, align=left, text=black]
at (rel axis cs:0.653,0.36) {D};
\end{axis}
%\end{tikzpicture}%

==> sym19_old_EV.tex <==
%% This file was created by matlab2tikz.
%%
%%The latest updates can be retrieved from
%%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%%where you can also make suggestions and rate matlab2tikz.
%%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
%\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
%\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%%
%\begin{tikzpicture}

\begin{axis}[%
width=0.951\picwidth,
height=.40\picheight,
at={(0\picwidth,0\picheight)},
scale only axis,
xmin=0,
xmax=2032,
xtick={0,500,1000,1500,2000},
xticklabels={{0},{.5},{1.0},{1.5},{2.0}},
xlabel={\footnotesize fiber length z, ($\times$1000 km)},
ymin=0.8,
ymax=2.2,
ytick={0.8,1.2,1.6,2},
ylabel={\footnotesize Imag($\lambda_i(z)$)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot [color=mycolor1,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	2.00047879800113\\
24.2	2.00093941388671\\
48.4	2.00122880947133\\
72.6	2.00040323984403\\
96.8	2.00002819456301\\
121	1.99731383213215\\
145.2	1.99576033087438\\
169.4	1.99405278746286\\
193.6	1.99181657738007\\
217.8	1.98948783442689\\
242	1.98804612885425\\
266.2	1.98809869281399\\
290.4	1.98940397145757\\
314.6	1.99466448365205\\
338.8	2.004096191737\\
363	2.01690501742364\\
387.2	2.0306814923397\\
411.4	2.04154291178201\\
435.6	2.04794204183147\\
459.8	2.04884219077436\\
484	2.04586265805136\\
508.2	2.04027783469443\\
532.4	2.03232190624315\\
556.6	2.02416886052765\\
580.8	2.01657245949202\\
605	2.00770656976567\\
629.2	1.99867350988286\\
653.4	1.99059831510371\\
677.6	1.98384943409108\\
701.8	1.97658935482461\\
726	1.96972923863557\\
750.2	1.96445358244004\\
774.4	1.96124573424119\\
798.6	1.96074898584297\\
822.8	1.96326492687579\\
847	1.96850366191207\\
871.2	1.97573274404634\\
895.4	1.98378487832923\\
919.6	1.99212555934468\\
943.8	1.99929375552147\\
968	2.00608864103165\\
992.2	2.01121668143502\\
1016.4	2.01514372327812\\
1040.6	2.01804805516395\\
1064.8	2.01953784906359\\
1089	2.01963027424644\\
1113.2	2.01816229662111\\
1137.4	2.01574260560164\\
1161.6	2.01238611886022\\
1185.8	2.00912535890317\\
1210	2.00399943816921\\
1234.2	1.99850498434518\\
1258.4	1.99328900398012\\
1282.6	1.99157121614016\\
1306.8	1.98895950754893\\
1331	1.9882756662492\\
1355.2	1.98650277461544\\
1379.4	1.98734747100376\\
1403.6	1.98801637395242\\
1427.8	1.99007194710938\\
1452	1.99352682503859\\
1476.2	1.99759463179274\\
1500.4	2.00209481919293\\
1524.6	2.0061852672152\\
1548.8	2.00935278458106\\
1573	2.00985064739854\\
1597.2	2.00768150768368\\
1621.4	2.00336594206029\\
1645.6	1.99834325844706\\
1669.8	1.99422898906004\\
1694	1.9928906022974\\
1718.2	1.99379273207847\\
1742.4	1.9963066663581\\
1766.6	2.0007823886856\\
1790.8	2.00367379485039\\
1815	2.00793961351654\\
1839.2	2.00971856599725\\
1863.4	2.01042095629703\\
1887.6	2.01116524947965\\
1911.8	2.01005373860932\\
1936	2.01024430765129\\
1960.2	2.00834433009949\\
1984.4	2.00697871042715\\
2008.6	2.00482769220877\\
2032.8	2.00330893112282\\
};
\addplot [color=mycolor2,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.99964541642523\\
24.2	2.00125821016011\\
48.4	2.00251992568754\\
72.6	2.00459365702464\\
96.8	2.0046479290888\\
121	2.00935926975658\\
145.2	2.01134988785696\\
169.4	2.01476993768174\\
193.6	2.01843277579414\\
217.8	2.02229554002765\\
242	2.02395157175508\\
266.2	2.02334016210537\\
290.4	2.02040379639033\\
314.6	2.01099091845388\\
338.8	1.99565893488389\\
363	1.97518695934751\\
387.2	1.95311403420309\\
411.4	1.93505885986134\\
435.6	1.92428382672352\\
459.8	1.92289778166662\\
484	1.92759359265144\\
508.2	1.93763747686213\\
532.4	1.95028912477918\\
556.6	1.96338439733101\\
580.8	1.97631131104609\\
605	1.98833966353104\\
629.2	2.00161901839698\\
653.4	2.01246126669014\\
677.6	2.02195566953217\\
701.8	2.03178230142494\\
726	2.04269796002987\\
750.2	2.05079464188108\\
774.4	2.05736335117368\\
798.6	2.06055425057813\\
822.8	2.0597777432389\\
847	2.05486410690534\\
871.2	2.04646700056443\\
895.4	2.03582137552256\\
919.6	2.0231526322675\\
943.8	2.01133445745307\\
968	1.9994637694058\\
992.2	1.98962142972771\\
1016.4	1.98190160594092\\
1040.6	1.97671469102104\\
1064.8	1.97528852545446\\
1089	1.97709667791353\\
1113.2	1.9836936959479\\
1137.4	1.99165069282458\\
1161.6	2.00156832830625\\
1185.8	2.00987541434958\\
1210	2.01856807214928\\
1234.2	2.02598539870854\\
1258.4	2.0323903604346\\
1282.6	2.02543441065797\\
1306.8	2.0203678557595\\
1331	2.00883655165779\\
1355.2	1.99787847786394\\
1379.4	1.98406258094934\\
1403.6	1.96919068958024\\
1427.8	1.95428024232752\\
1452	1.93972654327614\\
1476.2	1.9283394126327\\
1500.4	1.92229758989481\\
1524.6	1.92459427968044\\
1548.8	1.93713938913321\\
1573	1.9609558369851\\
1597.2	1.99370009947442\\
1621.4	2.02797475409565\\
1645.6	2.05796832277886\\
1669.8	2.07990521942002\\
1694	2.09325153902603\\
1718.2	2.09702846707913\\
1742.4	2.09269621003073\\
1766.6	2.08239274108196\\
1790.8	2.06885909227678\\
1815	2.05087682245094\\
1839.2	2.03628696396443\\
1863.4	2.02179816552781\\
1887.6	2.00946222610932\\
1911.8	2.0011461557418\\
1936	1.99059278020523\\
1960.2	1.98806688714536\\
1984.4	1.98353295422262\\
2008.6	1.98346404347131\\
2032.8	1.98165137125675\\
};
\addplot [color=mycolor3,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.99916822753693\\
24.2	1.99450540784645\\
48.4	1.99988410324245\\
72.6	1.99729328552356\\
96.8	1.99986736240572\\
121	1.99824596470956\\
145.2	1.99950045160139\\
169.4	2.0001517504505\\
193.6	2.0010224889962\\
217.8	2.00193948586331\\
242	2.00344736329716\\
266.2	2.0054959610051\\
290.4	2.00718635874645\\
314.6	2.0089903978335\\
338.8	2.01011621139363\\
363	2.01008701209902\\
387.2	2.00850555131991\\
411.4	2.00480350425737\\
435.6	1.9997853130334\\
459.8	1.99390590239062\\
484	1.98773066969909\\
508.2	1.98292284932584\\
532.4	1.97829477313259\\
556.6	1.9752974665919\\
580.8	1.97546640893823\\
605	1.97478069107722\\
629.2	1.97453335152901\\
653.4	1.97404211922304\\
677.6	1.97449730058438\\
701.8	1.97398393801503\\
726	1.97129733870551\\
750.2	1.96858510028032\\
774.4	1.96625318109894\\
798.6	1.96266717346064\\
822.8	1.96090711046487\\
847	1.96103138594125\\
871.2	1.96340591717341\\
895.4	1.96817652998502\\
919.6	1.97620878121334\\
943.8	1.98557821077009\\
968	1.99461556799061\\
992.2	2.00391245170963\\
1016.4	2.01001838054092\\
1040.6	2.01200385493136\\
1064.8	2.00857570296164\\
1089	1.99999776398155\\
1113.2	1.98508963010075\\
1137.4	1.96823222617726\\
1161.6	1.95222153514146\\
1185.8	1.93989240158647\\
1210	1.93772586528669\\
1234.2	1.93330331248334\\
1258.4	1.9413879177335\\
1282.6	1.95898957531359\\
1306.8	1.98382586197355\\
1331	2.01176098088827\\
1355.2	2.04494169403914\\
1379.4	2.077566063311\\
1403.6	2.10902692467163\\
1427.8	2.13757929259387\\
1452	2.15958851441452\\
1476.2	2.17172098565224\\
1500.4	2.16950149900905\\
1524.6	2.14953541982019\\
1548.8	2.10718141277603\\
1573	2.0433748068171\\
1597.2	1.95889191177248\\
1621.4	1.8712230220707\\
1645.6	1.80036801359901\\
1669.8	1.75649583693099\\
1694	1.73711688896182\\
1718.2	1.74085084879659\\
1742.4	1.75898119630646\\
1766.6	1.78701914593252\\
1790.8	1.82380527606384\\
1815	1.86021057488123\\
1839.2	1.89408537099091\\
1863.4	1.92327272611369\\
1887.6	1.95036562237709\\
1911.8	1.97289586467088\\
1936	1.99320991105939\\
1960.2	2.00536188990408\\
1984.4	2.01640100485628\\
2008.6	2.02366835791156\\
2032.8	2.03169494922566\\
};
\addplot [color=mycolor4,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.99911985279581\\
24.2	1.9995503728524\\
48.4	2.0036939012008\\
72.6	2.0062014591427\\
96.8	2.009028037412\\
121	2.01548306559663\\
145.2	2.0182352471582\\
169.4	2.0213192513273\\
193.6	2.02601158832984\\
217.8	2.02870656057908\\
242	2.03168622987723\\
266.2	2.02996016485364\\
290.4	2.02561867523883\\
314.6	2.01585052087805\\
338.8	2.00148606710161\\
363	1.98046741450451\\
387.2	1.9552429553621\\
411.4	1.9290136466847\\
435.6	1.90646626320804\\
459.8	1.89049807994214\\
484	1.88374866492886\\
508.2	1.88764054494198\\
532.4	1.89926065770614\\
556.6	1.91329520541307\\
580.8	1.9276222352801\\
605	1.94158641092411\\
629.2	1.95746456551093\\
653.4	1.97356234217461\\
677.6	1.98451269731656\\
701.8	1.99887539993048\\
726	2.01008712665986\\
750.2	2.02087916448912\\
774.4	2.02771112472239\\
798.6	2.03437488181555\\
822.8	2.03919060974825\\
847	2.03949135454496\\
871.2	2.03624451036796\\
895.4	2.03046112961256\\
919.6	2.01923688775265\\
943.8	2.0066425746639\\
968	1.99174549262238\\
992.2	1.97520634338912\\
1016.4	1.96241308442886\\
1040.6	1.95117420956375\\
1064.8	1.94570662630476\\
1089	1.94602791270062\\
1113.2	1.95118141688529\\
1137.4	1.96358228878803\\
1161.6	1.97389482304204\\
1185.8	1.99163933380636\\
1210	1.99613526102373\\
1234.2	2.00927760826028\\
1258.4	2.01469017668086\\
1282.6	2.01395617746216\\
1306.8	2.00622495501964\\
1331	1.99477384796125\\
1355.2	1.98176213705835\\
1379.4	1.96612668939995\\
1403.6	1.95300429235359\\
1427.8	1.94024305781068\\
1452	1.92914895034651\\
1476.2	1.92038095406895\\
1500.4	1.91481309654274\\
1524.6	1.91307000568723\\
1548.8	1.92066252561564\\
1573	1.94202124364936\\
1597.2	1.98273204986748\\
1621.4	2.03569882308225\\
1645.6	2.08471279212172\\
1669.8	2.11770948005868\\
1694	2.13458437740996\\
1718.2	2.13688087757022\\
1742.4	2.13049695146673\\
1766.6	2.11584594570839\\
1790.8	2.09587190048269\\
1815	2.0760171852184\\
1839.2	2.05841041734686\\
1863.4	2.04156333776908\\
1887.6	2.0243411281467\\
1911.8	2.0102662340446\\
1936	1.9949785428619\\
1960.2	1.98446937436751\\
1984.4	1.97501168114802\\
2008.6	1.96775843896625\\
2032.8	1.96257540717559\\
};
\addplot [color=mycolor5,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	2.00030918005814\\
24.2	1.9998812767043\\
48.4	1.99943016558594\\
72.6	1.99742741993811\\
96.8	1.99568355088062\\
121	1.99290180143428\\
145.2	1.99128190671181\\
169.4	1.98952254138659\\
193.6	1.98692827751637\\
217.8	1.98479491451301\\
242	1.98298538009445\\
266.2	1.98321700116746\\
290.4	1.98482499249682\\
314.6	1.98887278618416\\
338.8	1.99523195086331\\
363	2.00432196957217\\
387.2	2.01505628919414\\
411.4	2.02563845377423\\
435.6	2.03436370229199\\
459.8	2.04049173180632\\
484	2.0435886405472\\
508.2	2.04312829271015\\
532.4	2.04008894350343\\
556.6	2.03589271746974\\
580.8	2.03151111020076\\
605	2.02605219200746\\
629.2	2.0204481853773\\
653.4	2.01385361208437\\
677.6	2.00882188010697\\
701.8	2.00352799056827\\
726	1.99881805007712\\
750.2	1.99429852806644\\
774.4	1.99093931168833\\
798.6	1.988179289073\\
822.8	1.98635775388675\\
847	1.98623685901583\\
871.2	1.98730899564208\\
895.4	1.98917015915128\\
919.6	1.99250273665268\\
943.8	1.99613422648599\\
968	2.00033972887531\\
992.2	2.00514627036164\\
1016.4	2.00932468812294\\
1040.6	2.01370698795146\\
1064.8	2.01731650498112\\
1089	2.02035441190103\\
1113.2	2.02254755106248\\
1137.4	2.02323357848712\\
1161.6	2.02301180138825\\
1185.8	2.02041917653547\\
1210	2.01822938776077\\
1234.2	2.01284832194414\\
1258.4	2.00825749466934\\
1282.6	2.00247954351096\\
1306.8	1.99852077323652\\
1331	1.9942539170351\\
1355.2	1.99007611357107\\
1379.4	1.98807071144754\\
1403.6	1.98610048749185\\
1427.8	1.98567276433869\\
1452	1.98655763371362\\
1476.2	1.98904558749658\\
1500.4	1.993056848553\\
1524.6	1.9987151992717\\
1548.8	2.00522797842299\\
1573	2.01159406076948\\
1597.2	2.01689103904858\\
1621.4	2.02085140874664\\
1645.6	2.02274110514023\\
1669.8	2.02284393756508\\
1694	2.02125215162725\\
1718.2	2.01846489540127\\
1742.4	2.0151749672906\\
1766.6	2.01272693624263\\
1790.8	2.01012665390746\\
1815	2.00732910850138\\
1839.2	2.00602475605786\\
1863.4	2.00506115776716\\
1887.6	2.00457341274774\\
1911.8	2.00433329807686\\
1936	2.00433978697012\\
1960.2	2.00584098571892\\
1984.4	2.00499753706853\\
2008.6	2.00575647515995\\
2032.8	2.00494053366774\\
};
\addplot [color=mycolor6,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.00142488940388\\
24.2	1.0001308744554\\
48.4	1.00023135129429\\
72.6	0.998880964822876\\
96.8	0.998405552961182\\
121	0.997388102326844\\
145.2	0.997705802203437\\
169.4	0.996666671533494\\
193.6	0.99718003950667\\
217.8	0.99725432124726\\
242	0.999019036063448\\
266.2	1.00103083484898\\
290.4	1.00481265476868\\
314.6	1.00985228141709\\
338.8	1.01620735461409\\
363	1.02310144517559\\
387.2	1.02942445882886\\
411.4	1.0342518957874\\
435.6	1.0359742427631\\
459.8	1.03573335725095\\
484	1.03289823511858\\
508.2	1.02951239107604\\
532.4	1.02620597147895\\
556.6	1.02198340794013\\
580.8	1.01957602771891\\
605	1.01705358409925\\
629.2	1.01478510108538\\
653.4	1.0132789779511\\
677.6	1.01266311413995\\
701.8	1.01156447404113\\
726	1.0092794924961\\
750.2	1.00795518892017\\
774.4	1.00561748880921\\
798.6	1.00265689004854\\
822.8	0.998860175543436\\
847	0.995777768198393\\
871.2	0.992897670694633\\
895.4	0.990570263317761\\
919.6	0.989445064309411\\
943.8	0.989541274873059\\
968	0.990842668220244\\
992.2	0.992922692774688\\
1016.4	0.995717046690919\\
1040.6	0.998201678477201\\
1064.8	1.00076622189349\\
1089	1.00217438034863\\
1113.2	1.00347474435002\\
1137.4	1.00373781786708\\
1161.6	1.00410476585154\\
1185.8	1.00286814774696\\
1210	1.00238310577671\\
1234.2	1.00104887116759\\
1258.4	0.999858262907512\\
1282.6	0.999474157156182\\
1306.8	0.999002732211772\\
1331	1.00064050143262\\
1355.2	1.00160943689702\\
1379.4	1.00227137328989\\
1403.6	1.00440223565281\\
1427.8	1.0054312828928\\
1452	1.00672918518474\\
1476.2	1.00759715602088\\
1500.4	1.00862519761315\\
1524.6	1.00895321419133\\
1548.8	1.00941070245676\\
1573	1.00922710017601\\
1597.2	1.00876798669327\\
1621.4	1.00774273782393\\
1645.6	1.00612071211184\\
1669.8	1.00399134294284\\
1694	1.0014819384034\\
1718.2	0.999460606656715\\
1742.4	0.997802854470782\\
1766.6	0.997362110087863\\
1790.8	0.997523210559493\\
1815	0.998289500354634\\
1839.2	0.999864709158173\\
1863.4	1.00159701930455\\
1887.6	1.00349220037851\\
1911.8	1.00522153485561\\
1936	1.00645915626175\\
1960.2	1.00815337448467\\
1984.4	1.00879753955279\\
2008.6	1.00922749328375\\
2032.8	1.00907766914068\\
};
\addplot [color=mycolor7,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	1.00091168445516\\
24.2	1.0025116600805\\
48.4	0.998980488163806\\
72.6	0.998252374724628\\
96.8	0.994871631839534\\
121	0.99263128886352\\
145.2	0.991153293009808\\
169.4	0.988583465500412\\
193.6	0.985328729726204\\
217.8	0.983651136227787\\
242	0.981265728143244\\
266.2	0.979815789147637\\
290.4	0.980548078142441\\
314.6	0.9832624489912\\
338.8	0.989271997748236\\
363	0.9998504768892\\
387.2	1.01439618232368\\
411.4	1.03224474539883\\
435.6	1.04988213944424\\
459.8	1.06436305457883\\
484	1.07291910427597\\
508.2	1.07390451998081\\
532.4	1.06913578451853\\
556.6	1.06228268393282\\
580.8	1.05347857621958\\
605	1.04451545211251\\
629.2	1.03459342182908\\
653.4	1.0245808229288\\
677.6	1.01667958265345\\
701.8	1.00847457786996\\
726	1.00201400604145\\
750.2	0.997681778093239\\
774.4	0.994832128945779\\
798.6	0.992957453441231\\
822.8	0.992675511047404\\
847	0.993792870861278\\
871.2	0.996334729013127\\
895.4	0.999461864230711\\
919.6	1.00372335694356\\
943.8	1.00820325937097\\
968	1.0138641042598\\
992.2	1.01962399708022\\
1016.4	1.02534454141371\\
1040.6	1.0306423053719\\
1064.8	1.03556682590439\\
1089	1.03786611392612\\
1113.2	1.0393999543906\\
1137.4	1.03723168174597\\
1161.6	1.03502339846949\\
1185.8	1.02924153384712\\
1210	1.02555596639438\\
1234.2	1.01829452355436\\
1258.4	1.01229952468104\\
1282.6	1.00661902010378\\
1306.8	1.00431608377941\\
1331	1.00202830743831\\
1355.2	0.999211122977575\\
1379.4	0.998540841361129\\
1403.6	0.995301386323969\\
1427.8	0.994386557904614\\
1452	0.993315917299355\\
1476.2	0.99594175855079\\
1500.4	1.00128296572691\\
1524.6	1.01013413912978\\
1548.8	1.0215830178427\\
1573	1.03184480963709\\
1597.2	1.03718737910098\\
1621.4	1.03617574600709\\
1645.6	1.03057646751513\\
1669.8	1.02405449060247\\
1694	1.01710012674411\\
1718.2	1.01100157470098\\
1742.4	1.00524367678727\\
1766.6	1.00058272997054\\
1790.8	0.99754848787455\\
1815	0.995348801893576\\
1839.2	0.993750804884664\\
1863.4	0.994852552036869\\
1887.6	0.995846735593451\\
1911.8	0.997870360772621\\
1936	0.999846207994225\\
1960.2	1.00313913505267\\
1984.4	1.00551112069211\\
2008.6	1.01020158970203\\
2032.8	1.00972797941308\\
};
\addplot [color=mycolor1,solid,line width=1.0pt,forget plot]
  table[row sep=crcr]{%
0	0.998917725476889\\
24.2	0.998676569392953\\
48.4	0.999052145239412\\
72.6	0.998700768897541\\
96.8	0.99888059014803\\
121	0.998566882460038\\
145.2	0.997865845812933\\
169.4	0.996556677821467\\
193.6	0.995410799092191\\
217.8	0.993784903304277\\
242	0.992331583300863\\
266.2	0.990647933894601\\
290.4	0.989313932973561\\
314.6	0.988804691496009\\
338.8	0.989430227843047\\
363	0.991449654178552\\
387.2	0.994778954283235\\
411.4	0.998869423693104\\
435.6	1.00275307694379\\
459.8	1.00583655039935\\
484	1.00729200850106\\
508.2	1.00711296420361\\
532.4	1.00623416957173\\
556.6	1.00490019380556\\
580.8	1.0030244406973\\
605	1.00103327881326\\
629.2	0.999837686282222\\
653.4	0.998962464219593\\
677.6	0.998587619179723\\
701.8	0.99800185059746\\
726	0.997898496998282\\
750.2	0.998099223455786\\
774.4	0.998821661413634\\
798.6	0.999807007468694\\
822.8	1.00095862816606\\
847	1.00246676713341\\
871.2	1.00383701897695\\
895.4	1.00505646628576\\
919.6	1.00572746408451\\
943.8	1.00583144818611\\
968	1.00543294432176\\
992.2	1.00439989939794\\
1016.4	1.00312616365535\\
1040.6	1.00147371777784\\
1064.8	0.999805075788836\\
1089	0.998737526493514\\
1113.2	0.998120457687582\\
1137.4	0.998285848184625\\
1161.6	0.998235961580395\\
1185.8	0.999986770236498\\
1210	1.00094218010171\\
1234.2	1.00246475984036\\
1258.4	1.00334640111282\\
1282.6	1.00345527473114\\
1306.8	1.00289837309535\\
1331	1.00206004436262\\
1355.2	0.999992271430115\\
1379.4	0.99734491210054\\
1403.6	0.995830554018245\\
1427.8	0.993825660409294\\
1452	0.991989699765283\\
1476.2	0.990295340863369\\
1500.4	0.989710287303812\\
1524.6	0.989664394641513\\
1548.8	0.990817455266991\\
1573	0.993076837109604\\
1597.2	0.995933339306054\\
1621.4	0.998870516162954\\
1645.6	1.00199285165119\\
1669.8	1.00383617463761\\
1694	1.0052534326982\\
1718.2	1.00633289851519\\
1742.4	1.00671397251686\\
1766.6	1.00665470402772\\
1790.8	1.00580025169379\\
1815	1.0053192674955\\
1839.2	1.0049995074066\\
1863.4	1.00423879537981\\
1887.6	1.00307812300687\\
1911.8	1.0015930571259\\
1936	1.00067478602755\\
1960.2	1.00002503199154\\
1984.4	0.999061913808615\\
2008.6	0.997894827869781\\
2032.8	0.998058289977035\\
};
\end{axis}

\begin{axis}[%
width=1.227\picwidth,
height=1.227\picheight,
at={(-0.16\picwidth,-0.135\picheight)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
hide axis,
axis x line*=bottom,
axis y line*=left
]
\node[below right, align=left, text=black]
at (rel axis cs:0.735,0.34) {C};
\node[below right, align=left, text=black]
at (rel axis cs:0.278,0.34) {A};
\node[below right, align=left, text=black]
at (rel axis cs:0.476,0.34) {B};
\end{axis}
%\end{tikzpicture}%

==> sym19_spectrum.tex <==
\begin{axis}[%
width=0.951\picwidth,
height=\picheight,
at={(0\picwidth,0\picheight)},
scale only axis,
xmin=-2.5,
xmax=2.5,
xtick={-2.5,-2,-1.5,-1,-0.5,0,0.5,1,1.5,2,2.5},
xticklabels={{},{-2},{},{-1},{},{0},{},{1},{},{2},{}},
xlabel={$\text{Re(}{\lambda}\text{)}$},
xmajorgrids,
ymin=0.5,
ymax=2.5,
ylabel={$\text{Imag(}\lambda\text{)}$},
ymajorgrids,
axis background/.style={fill=white}
]
\addplot [color=mycolor1,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.163969397118027	2.17420430844196\\
-2.08873979156066	2.0643924847237\\
2.01877312046989	1.99835927639309\\
1.17242693392756	1.95211053683202\\
-0.876641560121318	1.88659135637845\\
1.99975761488998	0.992463035310838\\
-0.996256049300674	0.984594591041997\\
0.938695155601286	0.934566208571093\\
-2.09383423691691	2.07747732573923\\
2.00114058989044	2.03979034868691\\
-0.0506650635613551	2.0280248115699\\
1.09087195812579	1.93671885254679\\
-0.892914245583745	1.90170401986282\\
2.03781988599929	1.02579141354744\\
0.991527017321445	1.00664346436786\\
-1.04625720230132	0.978192972175544\\
-2.01023541388339	2.18772242276195\\
1.06805973415589	2.07103609817841\\
2.01816987008751	2.00704309485894\\
-0.921566910955535	1.95166616065708\\
-0.204896155946545	1.8726681621418\\
1.06865792001288	1.0335613423689\\
1.99056238525063	1.03238591880088\\
-1.03476929975893	1.00295427785679\\
-0.895693911706809	2.09259702210123\\
0.985181699845049	1.99753223099042\\
2.03905283808353	1.95760681670965\\
-0.00190852629538476	1.9008485904093\\
-2.10716274528382	1.88075089735904\\
0.992704109314618	1.02935356093997\\
-1.03636201954523	1.0002830222755\\
1.97337713664953	0.976549493464086\\
1.23938818688924	2.25735043139072\\
-0.954373647107651	2.10190719099447\\
-1.94786968480688	1.96662869940834\\
-0.21641590412144	1.94811444200652\\
1.88329085677962	1.93677131295579\\
1.98565883615724	1.02765347065479\\
0.990362416081498	0.955598958870402\\
-0.93212883284584	0.950594805547942\\
1.23938818688924	2.25735043139072\\
-0.954373647107651	2.10190719099447\\
-1.94786968480688	1.96662869940834\\
-0.21641590412144	1.94811444200652\\
1.88329085677962	1.93677131295579\\
1.98565883615724	1.02765347065479\\
0.990362416081498	0.955598958870402\\
-0.93212883284584	0.950594805547942\\
-1.11844355980982	2.28756231996351\\
0.812424989863588	2.26581146688913\\
2.03941672012055	1.98791240136435\\
-1.91855086385103	1.82359994846407\\
0.0163047801554034	1.72156774739656\\
1.13180654210634	0.990059173131226\\
-0.9427788787514	0.981688710105441\\
1.98710339899491	0.97836385502364\\
1.05373126374106	2.15027222255313\\
-0.997366367727694	2.03826536824599\\
-2.01617116557344	2.0253644404075\\
2.01083520405867	1.95000465907632\\
-0.00234439548607928	1.86150492205202\\
-1.04498174332845	1.03260164204163\\
2.00208273885855	1.00707629609067\\
0.977173558386141	0.972011158780904\\
-1.96744843242543	2.15878989734394\\
-0.0803985230959322	2.09515691908635\\
2.07050072661686	1.93588940586607\\
1.02832302323027	1.83662389892884\\
-1.035353061611	1.83193846160385\\
-1.07293712592995	1.02198870129279\\
0.928358852814337	1.01751185865935\\
2.04482338702366	1.01127325556248\\
1.18640827440992	2.18812105714777\\
-0.941642264303998	2.00657253306253\\
-0.127593230218861	1.97408073914403\\
-2.05568076648841	1.94377956746977\\
1.95608976144441	1.90691482242342\\
2.03341351583405	0.994252313722539\\
-0.981102854363903	0.980043540918084\\
0.968655978381953	0.891679804497807\\
-1.87908407228839	2.13371282475304\\
1.98997301472951	2.0613831539292\\
0.301993054680115	2.04723478805982\\
-1.26065585860535	1.81934527337731\\
0.877162823644109	1.61688305626164\\
0.959382054049191	1.26338549664419\\
-0.980909012259139	1.05388720446777\\
1.99983344474774	0.964482485051917\\
-1.99928753051654	2.15068313309148\\
2.01703772253809	2.02888388973697\\
0.952120913231172	2.01884838675244\\
-0.0163667891255371	2.00563056572086\\
-0.991448885289834	1.81120249248661\\
1.98644786748719	0.995371805713362\\
1.07301495559218	0.988079679594771\\
-1.02355271411361	0.985690350010229\\
1.25171430675563	2.07552131886886\\
-0.144336733395735	2.07210262670246\\
-2.03822963674197	1.98429419411111\\
-0.894747025407422	1.94006103277924\\
1.94922308018432	1.87786650524821\\
-1.04192296126905	1.02967358600629\\
2.02886567581895	1.00740602618016\\
0.86684355331143	0.920781957130537\\
0.0400735492281658	2.10049661379191\\
2.0391103566878	2.05352691032923\\
-0.966683981389365	2.00511611820858\\
-2.05076848245892	1.99725667724346\\
0.976507771762224	1.78954750651923\\
0.98603137296296	1.03833549540421\\
2.03219134249664	1.01346557329746\\
-0.992663391490912	0.960457492251725\\
-2.01729027487983	2.0375389563321\\
0.901589646231834	2.02125026079657\\
-1.03461698015506	2.00719655650302\\
2.03485491861126	1.98117372629319\\
-0.0233246906495392	1.93314234047468\\
1.04429411020876	1.03996282814347\\
-0.985731483698448	1.0012071016437\\
2.00198649845451	0.99115922193614\\
-0.0124375597090546	2.09835926838229\\
-1.08399363940976	2.07745760082526\\
1.98291185473352	2.06305676510055\\
-1.96266699000039	1.8803682013347\\
1.1602938406475	1.79628249768646\\
-0.936486339953245	1.04238292766378\\
0.916014893617386	1.02801948255964\\
2.02908135523794	1.00167359563762\\
-0.0140114547042634	2.07794370429801\\
-1.89510348882842	2.07518882552832\\
1.99015056798529	2.06114493075858\\
1.07565768008955	1.89436199274827\\
-1.08791081381392	1.86007664275902\\
2.01502028676429	1.01828897401556\\
-1.01848408473061	1.01748489213383\\
1.01204938780407	0.994396153811177\\
0.171711986886605	2.11689720329156\\
1.9057716680089	2.03094662891734\\
-1.95497952066003	2.00851355846659\\
-1.04083814999129	1.94647468305342\\
1.0858522219511	1.88720736813558\\
-1.05931792945057	1.05640307589846\\
0.879058921215744	1.04068547453254\\
2.01243002397345	0.999786344294457\\
2.02479371832699	2.07233223449522\\
-1.02742286727974	1.98093485298406\\
0.96744226960836	1.97719354327136\\
-2.06254959996806	1.92587011350416\\
0.109187704014733	1.90094885704667\\
1.00849542615325	1.06380567047149\\
1.99397311414707	0.990701151939384\\
-0.971695929993526	0.967339303100511\\
0.0656850420593284	2.20709093296357\\
1.87763662762333	2.06348986627958\\
-2.0212847510054	1.98950184104714\\
-0.991476459450719	1.92885830100729\\
1.21274179954516	1.90005777602528\\
0.869767093527667	1.01290948923065\\
-0.993439010691468	0.98481661342386\\
2.01211616933801	0.980788894520601\\
1.06967219083065	2.11564437732544\\
-0.854351759847191	2.01269150948394\\
-2.08141241099225	1.9802984092909\\
-0.218809783646405	1.9568170845269\\
2.0368775917974	1.93099793371719\\
2.02102501669593	1.01619819579925\\
-1.02748909882042	1.00184466881301\\
1.03328490879502	0.877347146361911\\
0.0470823828971756	2.17056129088506\\
-2.02317838004655	2.04063714497448\\
1.98315258471102	1.9943199075964\\
1.00770362637255	1.88622994283532\\
-1.01560931813439	1.85907455347146\\
0.97915027873241	1.00999990722519\\
2.04747776454632	1.00304241537707\\
-0.999265763671565	0.957831386151151\\
1.04510160261317	2.18454733678447\\
-2.01719323081477	1.9896386260108\\
-0.189955225739422	1.94464799502226\\
-0.929315706066119	1.91983857931753\\
2.03027536369784	1.90646590969101\\
2.00052007545819	1.02358455433914\\
-0.951329914205407	0.961999423588616\\
1.05175260283529	0.916916925808366\\
1.0962558680805	2.07604089790032\\
-0.0664622655886428	2.07122479215779\\
-2.00178854677379	2.00487385895482\\
-0.974388720639577	2.00231522379481\\
1.95626969728576	1.96586307001922\\
1.98243917006992	1.0262775225259\\
1.00831826551986	1.01085041676814\\
-0.984862007372219	0.969538920149115\\
0.103530236037995	2.16837947093801\\
1.91625781604195	2.0870181255506\\
-2.00016187573591	2.0281920658247\\
-1.03489847871786	1.81943510656547\\
1.1609585009408	1.75778515242659\\
0.848208963888974	1.07457350722519\\
-0.990415858382019	1.07207479563529\\
1.98526859430861	0.943076052857685\\
-0.111632763019421	2.2170503677651\\
1.89614787545792	2.04804776551556\\
-2.05082374874554	2.04501650092251\\
1.27411673918335	1.83619255246828\\
-0.842671291462086	1.82599452699654\\
-1.06363690217111	1.02411833864015\\
0.838450283123963	1.0016729672404\\
2.01573478829033	0.966096577681013\\
-0.0545778410434227	2.1140925838463\\
1.9600679155393	2.04295918241332\\
-2.06849035928096	2.03307901269448\\
-0.929915322215527	1.95789170510504\\
1.04698734527094	1.90214274306748\\
1.00747998330413	1.01907730718704\\
-0.992909072914916	0.993901510482124\\
2.01274236074443	0.992637507973143\\
0.884126813471347	2.06733362340887\\
-2.00211146885151	2.06095411158713\\
2.06964484198338	1.97600245420647\\
-1.06115540928931	1.94545919039152\\
-0.0141857932322435	1.90885950610765\\
-0.946032353538727	1.01627070981954\\
2.00434849555551	1.01454758817287\\
1.06867062870995	0.993221414714465\\
0.178003189912025	2.10714145364675\\
-2.00633601186596	1.98287206504135\\
2.02240189566518	1.97485135889437\\
-1.08219852351716	1.89207162554984\\
0.990286297823628	1.81751394932133\\
-0.979454586137502	1.06651045252643\\
0.892738352484191	1.05044943383478\\
1.99173954400101	0.999613427333166\\
2.09692949718145	2.02734687742464\\
-1.89837557136375	2.00780069410431\\
-1.11651059724856	1.95682572984994\\
0.87938433368358	1.884673353848\\
0.0152761303783986	1.84678683100228\\
1.05006237881625	1.10080246614526\\
2.0322979587385	0.998811683576127\\
-1.00690366831218	0.996824401731471\\
1.0704416739765	2.0355962285232\\
-2.03602639558094	2.03521171583063\\
2.0137150195737	2.02550773495217\\
-0.862560200342867	1.96900225461565\\
-0.220670718341801	1.96118485871724\\
-1.02571269167239	1.02812813641147\\
1.98243616315736	0.985243888766432\\
1.01626681130955	0.92521472715517\\
2.05784767422051	2.08715717628665\\
-1.98635673155099	2.05025271114527\\
-1.02140805152437	2.02843994618277\\
0.00604165008866723	2.01826860132144\\
0.897570942192983	1.79805426664476\\
1.06010092800804	1.04822076504343\\
-1.05734833193694	0.999865711384937\\
2.00840183933356	0.991370895725253\\
0.154791676337601	2.07111148169634\\
-1.86975234316023	2.04809424852226\\
2.03999052317217	1.98848790737411\\
-1.17846408258227	1.94758768341319\\
0.80579767249167	1.89165579857299\\
-0.968350827031611	1.05693679928312\\
0.999739668064874	1.0308154064425\\
2.011219420675	1.00137959034543\\
-0.142963589266625	1.98916422799424\\
1.07846030184028	1.98318437776533\\
-2.13821800152476	1.95868720695965\\
2.0253409859907	1.95377494178551\\
-0.851142283570692	1.89487434988594\\
1.01191982646477	1.00011964213903\\
2.00481896107942	0.993986022706208\\
-0.993602141407939	0.988115436716035\\
1.03279994690288	2.06062503508129\\
-2.04695481393021	1.98572092439275\\
-1.02727286202244	1.97356552784763\\
1.99250847668836	1.97184740254451\\
0.118428846774932	1.9511969081578\\
1.00922520078238	0.999521171861277\\
2.01461761163108	0.996509873213804\\
-1.00364874836028	0.947065613356954\\
-0.982131996829199	2.06625987568988\\
1.93604140075199	2.05332672418254\\
-0.0659060829837482	2.02595232955545\\
1.17496167052731	1.97892536139565\\
-2.01606029315781	1.95490427041221\\
2.02261372272208	1.01010121685385\\
-0.986562014341071	0.977893279965137\\
0.983628077355822	0.944218860344115\\
2.04571287619404	2.06561807247628\\
0.177311540581921	2.05422594933478\\
-2.11633306126717	1.99717731646567\\
-0.982716054545308	1.99558596711365\\
0.858606528067402	1.66009981105203\\
0.982038107642962	1.15606664484206\\
-1.02025286341268	1.01078378918845\\
1.98895242932668	0.952773876197886\\
1.07869471406433	2.17640881494697\\
-0.926694257598145	2.11447224968508\\
-0.0478747923780179	1.98755377761003\\
-2.05700977785716	1.92497088845556\\
1.95490411207363	1.89363532092204\\
2.02837666922516	0.998037454400085\\
-1.00003025161936	0.981238937584526\\
0.952925295869638	0.939444622561078\\
0.840524039369256	2.25072608891163\\
-1.15214992042137	2.12384208682031\\
-1.91890459091331	1.95543458712258\\
2.10783675776535	1.92932640974987\\
-0.00120786816332354	1.71273865548194\\
-1.00686115175405	1.03045520918543\\
1.98930895073441	1.00260018699537\\
1.10385671415074	0.956027357884115\\
0.847614387572261	2.12087426119866\\
-1.96809641755451	2.05474382323274\\
2.01090258602975	2.0025886433612\\
-1.1082609276807	1.97038024249229\\
0.178048067836521	1.69956890369855\\
1.09666072842366	1.12338710080527\\
-1.04367962762676	1.01774290921768\\
1.95322521022114	0.976958839254004\\
1.97552026167687	2.1291509864515\\
0.0948926907014767	2.06571481904787\\
-2.03196999856563	2.02947695683874\\
-0.963109614477674	1.93524936811117\\
1.11389558673307	1.52697463917825\\
0.86382847100673	1.31459089073274\\
-1.04599212736434	1.0476305336315\\
1.98391395127374	0.978956314803633\\
2.00235874405895	2.06025872676882\\
-1.05799132209198	2.04559350697496\\
-0.0236717863591411	2.01577831747424\\
-1.91675360100329	1.94198571560346\\
1.1592952122323	1.92665327641143\\
-0.988870233714368	1.03700303472949\\
1.98613122563046	0.987954273228938\\
0.901416698775773	0.976460282991509\\
1.15720556557477	2.08718259233664\\
-0.00716027606206998	2.05081892255126\\
-1.09318830990951	2.01935735504725\\
-1.90494332372489	2.0028181042593\\
1.95845990384696	1.93241993347038\\
2.01178389438764	1.01259870767343\\
-1.00019339466186	1.005808635833\\
0.91253436334268	0.907491388997548\\
-0.0212388443792351	2.13436351240539\\
-1.92650117576179	2.02168383896251\\
1.91983494334186	2.02021170314477\\
1.13118036313684	1.99360227692107\\
-1.07465447412601	1.94239815966867\\
-0.961752053305373	0.993282517364333\\
2.02290789951034	0.979504685902487\\
0.947396215709611	0.955345095126188\\
2.00243627089987	2.0360582274717\\
0.924548521322001	2.01857115961563\\
-2.08291578069628	1.98469073963492\\
-0.978159124291464	1.97745999128185\\
0.139009141577517	1.82559895369635\\
1.05891908377469	1.12361205164912\\
-1.01416155981415	1.04130009658326\\
1.96741337332147	1.0291947731351\\
0.0689680053741164	2.04108991637462\\
1.92636902618165	2.00933110156641\\
-1.09236038371822	2.0083880967613\\
-1.92918385350203	1.96898252246628\\
1.14933826866103	1.93856018480073\\
0.909033459451969	1.06491148213484\\
-0.972249103737544	0.99965488489732\\
1.99713132769889	0.980763244647383\\
1.9797994779835	2.06623803785995\\
-0.995847445484625	2.02378363906756\\
-2.00680488642391	1.9832367758607\\
-0.0310465971619598	1.96289892055405\\
1.18937380983511	1.83884852101509\\
0.870069423615038	1.03514154285261\\
-1.0416728990911	1.00303443316277\\
2.00226766223977	0.956833159095324\\
0.0490473504581535	2.13980074606428\\
1.96749526566115	2.09060341813532\\
-0.914641870727618	2.01352868286116\\
-2.0422441617777	1.94913020002221\\
1.11966044952796	1.82298083037634\\
0.903957322328079	1.0984747076839\\
1.95042021931727	0.991054395474513\\
-1.00399883480834	0.989171887063719\\
0.186652029386461	2.10429228556613\\
1.9613233992591	2.05790318966128\\
-1.069016071527	1.99608917446013\\
-1.99295764303097	1.92061760097154\\
1.09443375692627	1.85339410190489\\
0.857455774946971	1.0340030284232\\
-1.00989318126233	1.00877643440975\\
1.9926747403059	0.922865832926926\\
-0.260141784189191	2.17550567517126\\
-0.864510722164861	2.02298839946038\\
-2.02434694953871	1.9980858404387\\
1.96580452203152	1.95339322950799\\
1.19109544256531	1.93936323427543\\
-1.00383182898142	1.02132903632062\\
2.02211209284928	0.969847171237893\\
0.911835834425649	0.909186070445086\\
0.141346016982356	2.18291210001383\\
-1.02763624025439	2.04574503920978\\
2.0545565737757	2.02438439910777\\
-2.00807461241051	1.9503000903592\\
0.879920477727909	1.88074248268316\\
1.9908867419703	1.04913531984322\\
1.01554290680894	1.00838842015109\\
-0.961859561985299	0.982812249600149\\
-0.0820838834972888	2.23272947387989\\
1.1058066871424	2.0652714526111\\
-1.98416716130954	2.01516070212179\\
1.99261387994124	1.88056236567417\\
-1.04252587629336	1.85393430357621\\
-0.939998871692375	1.0466708204612\\
2.02149766044656	1.01944897676288\\
0.936813683071731	0.879575594151368\\
0.927084388560492	2.07540737186586\\
-0.936318774360646	2.03279591112629\\
-0.000595290928559522	1.98834928354954\\
-2.08371960476164	1.97882878231489\\
2.04979444242846	1.94020641311438\\
2.05151246846438	1.03500620307473\\
-0.988069040117967	0.979450525219891\\
1.01781865417157	0.925911505225301\\
-0.0742399372418532	2.0941341078059\\
1.98922059780749	1.98479192912005\\
-0.905524549312643	1.96728038096797\\
1.04459938426885	1.96498544944959\\
-2.06785107426229	1.96476610133243\\
2.02454077924462	0.991104757033242\\
1.01505963416757	0.983181116020383\\
-1.01644687292444	0.951050913174551\\
-1.11981484798436	2.09074112351777\\
1.01829507396977	2.05254860314657\\
-1.93205094099888	1.9782924184168\\
-0.00665249603703195	1.96767638819935\\
2.01207605705944	1.87655397509813\\
-0.996124050668062	1.01824708288561\\
2.04084166907631	0.963435583792823\\
0.918807921136174	0.92404252719209\\
1.0533029457311	2.22648508481361\\
-2.08132440031964	2.14278322847749\\
-0.232246337365265	2.05686072492129\\
2.00562119496588	1.85976772250291\\
-0.786271075538271	1.85903969867446\\
2.00552838890732	0.999506633137727\\
-1.05414631448096	0.985472752573737\\
0.994690498998121	0.918739455420263\\
-1.06057911032227	2.03381123526258\\
1.99897372833607	2.02190093423755\\
-1.96595247088642	1.98276371684229\\
0.900985753627549	1.9372185082924\\
0.133843304381952	1.92620208942939\\
1.03692220520934	1.0726092465776\\
2.00986186281481	1.00585785898042\\
-1.01954155534798	0.988779145947189\\
0.0627712833284287	2.12253406602918\\
1.99748635421843	2.05098605064767\\
-0.987529904677468	2.01166875307322\\
-2.06609688388772	1.91201145753259\\
1.14031961239683	1.8137117776556\\
0.90587802964804	1.00003210103167\\
1.99294369600714	0.982091733652686\\
-1.00157899678886	0.981743492000569\\
2.04008048134951	2.01011104097626\\
-2.06996462143805	1.99415282220596\\
-0.982858424241094	1.9717480498048\\
0.243273898921132	1.93430447341066\\
0.776454409937919	1.82829744496711\\
1.0214338946945	1.18574382443726\\
-1.05844024714813	1.01070490715964\\
2.00389935092746	1.00959519525483\\
-0.00709944933482581	2.06626592893447\\
1.95607646927999	2.02239521890265\\
-0.918705990056081	2.0162033434904\\
0.990775958297093	1.92799946837959\\
-2.08071338180902	1.90999546930035\\
1.00208048286811	1.05932191342448\\
-0.943343965071691	1.0017683143672\\
2.00344259467395	0.963777198752338\\
1.08958076285564	2.29484255704742\\
-0.918489455446888	2.10691013124706\\
-2.056970873222	2.04238080955946\\
2.03920332548472	1.88156706935292\\
-0.183795598831453	1.82660390966649\\
1.98733577091658	1.02090466229813\\
-1.0343998092783	0.961889861731957\\
1.05207282024354	0.905664241058715\\
-1.94819751837442	2.04816039626877\\
-0.0225633490811065	2.00463349838114\\
2.02531462798613	1.99777573805618\\
-1.06645895785721	1.98406248553383\\
1.08412916863495	1.84905415283951\\
-1.03501272410059	1.03612443068566\\
0.913365355024496	0.999643757996661\\
1.99910810591351	0.973383164341731\\
-2.11253954793452	2.08076098329569\\
-0.174539521907408	1.97740842058023\\
-0.852337057546257	1.96685852573351\\
1.05689968781197	1.93951936278763\\
2.00157541994207	1.93038117931205\\
0.936967719923404	1.04591563802074\\
-1.02570827209745	1.02600623644547\\
2.0209023462298	1.00406181366052\\
0.933197520808269	2.23956797209317\\
-1.99579425570633	2.03429168598542\\
2.05390630872727	1.95841956280849\\
-0.0291744929480828	1.94840072923293\\
-1.01287507693543	1.94198352460025\\
1.99804697957774	1.0500204993404\\
-0.968081044310559	0.982396168411454\\
1.08820658231027	0.928538429941681\\
-1.9151072019094	2.10274761002268\\
0.727301370947189	2.04436697974331\\
2.08656507798095	2.03291728150511\\
-1.19313024646186	1.92533788337083\\
0.259337374949247	1.88065546766517\\
2.0065326307889	1.01351123188065\\
1.06210221352975	1.00118739662886\\
-1.00566913602937	0.993676182273234\\
1.95922929243224	2.14112613407982\\
-0.887322152287041	2.11670875636398\\
-0.0507264923065842	1.98248105078456\\
-2.0748664399331	1.95947852267761\\
1.1074898154481	1.78633362457602\\
0.978210801799406	1.10450117662609\\
1.99811662015045	1.01448856687233\\
-1.01141965562637	0.985856625773\\
-1.09198795783105	2.07608745733365\\
1.98080120229031	2.01766587609215\\
-0.0545596392045	1.99634337814533\\
1.0755740503001	1.98694012880256\\
-1.9077771127622	1.9640103352798\\
-0.966943074629258	1.04095983767398\\
1.97861901333214	1.01234772661738\\
0.989026513306155	1.00049880690997\\
0.907042493287574	2.19917263954512\\
-0.97813972892935	2.14824873756562\\
2.05242499490329	1.93093874415572\\
-2.04118544636247	1.93001460168131\\
-0.0516262670880998	1.78387160634774\\
2.02304785255097	1.00591666813369\\
-1.02606109081643	0.988687517821304\\
1.09784821269782	0.943433983776055\\
0.032729194719018	2.12873659444449\\
1.94356701478806	2.09887824270405\\
-2.08442817524928	2.07207520902287\\
-0.948515917180441	1.83807940391019\\
1.28298876317859	1.72370651647061\\
0.800067282468168	1.03427841591771\\
-1.06272062514352	1.01523558628802\\
2.01848306678783	0.969668905071545\\
-0.973550242856194	2.03402054308718\\
-2.0118315114156	2.03231999553618\\
2.00303512712289	1.97803761745203\\
1.05698850776885	1.9651209614824\\
-0.120249803955427	1.96429490994602\\
-1.00259617794524	1.0391468890689\\
2.00981272420418	1.00531925289659\\
0.97056405047178	0.997799778492637\\
-1.92238062582882	2.10813324101156\\
0.983079090805539	2.02964803755372\\
-1.04754082545411	2.00312153170872\\
2.04896121717311	1.9965904323307\\
-0.134025287641893	1.82680758402241\\
2.00636327966942	1.04121438162942\\
-1.01440899712289	1.03392239575855\\
1.05141652643068	0.992701883530594\\
-1.92288808943284	2.01307545242906\\
1.89857560213094	1.98481574268375\\
0.013085628930633	1.96279738634897\\
1.22194429778459	1.88306581281569\\
-1.03490251270363	1.8794022938364\\
0.877229746238287	1.09227431128746\\
-1.07640099594051	1.033800140092\\
2.02252537391931	0.946970216794634\\
0.896305873344449	2.06429369162335\\
0.0380501886621561	2.00395710522705\\
-1.93618204697267	1.99982513956816\\
2.06621988187906	1.96803356726645\\
-1.1067843266717	1.961648617921\\
2.01916344895272	1.02290810340876\\
-0.967341798834352	0.962796857549028\\
1.06137515212044	0.914505119897999\\
-1.90038726409462	2.07042498441795\\
0.0395411606719038	2.0392711624955\\
2.01218133522	1.96928169822743\\
1.00636607114128	1.96836175488054\\
-1.17246517884333	1.95866934783723\\
-0.980734803871271	0.998444566189019\\
1.99575755174642	0.992615803623877\\
0.942277210170234	0.973397593833441\\
0.0168574886053644	2.22193804873168\\
1.95788382569206	2.11209588369092\\
-2.04353714943441	1.96624834195818\\
-0.889102812541006	1.93962291503923\\
1.2089876177282	1.72834818111843\\
0.832244749966063	1.04770060702118\\
-1.06273821159374	1.01974468722037\\
1.98266224483308	0.981515759642967\\
-0.015541708481766	2.15670945118222\\
-2.0569319425693	2.00965786183601\\
2.03055883841388	2.00749795170881\\
-0.976438792158563	1.90061269361511\\
1.07190182836347	1.73532450759546\\
0.887090320624273	1.06162188096312\\
-1.01028581457993	1.03018423911595\\
2.02363334583645	0.96222775949604\\
-0.228993899775348	2.04438965072996\\
-2.0890113968478	2.02904044441357\\
1.98985594816022	1.9969162428305\\
1.22387590668634	1.90548619248528\\
-0.809167729297084	1.85346444780406\\
0.946687093826565	0.994957525030462\\
-1.05105842348173	0.988708942114907\\
2.00675399785541	0.974965159895814\\
0.113874972026859	2.01648972352088\\
-1.99908955284331	1.97878308721064\\
2.07917394140946	1.97652805195255\\
-1.0467569123378	1.97228186392165\\
0.847145300118901	1.902016033666\\
0.992948275535513	1.03910989975237\\
-1.01450784252275	1.01846739819871\\
2.02835971117095	0.991080847534102\\
1.30825381045606	2.15304945576027\\
-2.06014147328268	2.07379641653707\\
-0.850006869867978	2.01245630001238\\
1.8773466866614	1.94356187033354\\
-0.212891377831454	1.882029165492\\
-1.06478113367539	1.00325932372298\\
1.98592601288815	0.963849710451961\\
0.956446344217058	0.938135262552775\\
-0.904789860163838	2.04607887739736\\
2.00190084786579	2.00541953704571\\
-2.10039992746387	1.9702103735262\\
1.07381580958352	1.96413754822671\\
-0.0185947338565123	1.90443557672403\\
-1.03819354053743	1.03478708437617\\
0.966906156689637	1.02900702251309\\
1.9966368995132	1.0089371833051\\
2.06697343817879	2.06471937518263\\
-2.00962324855444	2.062155730197\\
0.123616672468744	2.00923808840553\\
-1.03599694895572	1.91294635187616\\
0.80722141961017	1.87131918791338\\
1.06682751552866	1.06204292628342\\
-0.987878807937566	1.01473775789987\\
1.97962377131815	0.980712719583809\\
-1.17226954825548	2.10777409645106\\
2.05973725891019	2.03508534140217\\
0.896982387768974	1.98429375932627\\
-1.85773650071503	1.94294536750769\\
0.089497880355826	1.84797547228399\\
1.03446788850776	1.07339361951832\\
-1.01541217771575	0.988668362654022\\
1.97681552000798	0.976325048448906\\
1.10651608268908	2.11389936949006\\
-0.0351215644152529	2.07989733731159\\
-1.91074475106818	1.96993802155912\\
-1.13506340137126	1.93076827188146\\
1.99679870899633	1.90342279617739\\
-0.967505091091284	1.04871988291181\\
2.01271384593611	1.01215041636533\\
0.953676392495979	0.912226129823988\\
-1.15634081248371	2.18407828807757\\
2.0371468205428	2.1609017605444\\
0.176558277454128	2.02506292115421\\
-1.92355727204196	1.91326774576429\\
0.9681026547012	1.79126665779522\\
0.961661272276642	1.0601476515565\\
-0.977763600843796	1.01450471741417\\
1.98474970370195	1.00064470498913\\
0.00422503839743178	2.11371503031421\\
-2.08262807832222	2.08662729118355\\
1.98448678707164	2.00804718991437\\
1.13014171300065	1.79508673529398\\
-0.958466247181012	1.79339840079688\\
0.886755370965912	1.06208334324338\\
-1.01871855759475	1.00883412312996\\
2.01730118816386	0.982023731153772\\
-1.96163204680287	2.11296330371548\\
-0.014266582889786	2.10878021835879\\
1.96016232833479	1.99583556908937\\
1.06215256962716	1.90812330450099\\
-0.981867768239318	1.86600667476215\\
0.97090201218922	1.01505155328596\\
-1.05111142492452	1.01031660914579\\
2.00881432346847	1.00577643244347\\
-0.0415858344448865	2.19976128239053\\
-1.97517671602029	2.09424238404684\\
2.02223170506026	2.02836962110567\\
1.03959241121604	1.94637211461684\\
-1.03077431358174	1.89725917026677\\
1.99362530171092	0.997232851035206\\
-1.00049801827583	0.969035353350984\\
0.993424246436842	0.928195734331615\\
0.976500801544404	2.09968194275136\\
-1.02615495110649	2.09799250828607\\
2.04780995978583	1.97991559120755\\
0.00547281861538005	1.95363491156796\\
-1.98871363893039	1.95192920575658\\
1.97597783431667	1.00804262587373\\
-0.994513542107768	0.970546764573271\\
1.00633660019779	0.948655072345725\\
0.142457794080789	2.26952315506779\\
-2.01662176626034	2.07541772426244\\
2.0279090877195	2.03319492989748\\
-1.04458566788773	1.80742314377022\\
0.962590027110014	1.67939187671432\\
0.946199718837303	1.10551753573315\\
-1.02865700216094	0.984599025450049\\
1.9863713250277	0.967441384884469\\
1.1821489203659	2.10566480890702\\
-2.03238819799227	2.05686529099133\\
-0.149166894509893	2.05297912550913\\
1.92375470024862	1.95125415022159\\
-0.906293169076709	1.91118042568771\\
1.95550109251536	1.01681030137553\\
-0.961764553423377	1.01117524115813\\
0.988363393741064	0.990227782250629\\
-1.00002513169968	2.11693589924452\\
2.02481888294628	2.0678248580616\\
-2.04622441180492	1.90040430959106\\
1.03585941727096	1.89279141290888\\
-0.0278712229052426	1.88053863417476\\
1.00851726682729	1.00993683424135\\
2.01226949965836	0.980866767678779\\
-1.00298655288552	0.975105594015276\\
0.956105471303473	2.13330027627621\\
-1.04150871628776	2.03636372015187\\
2.02977051392822	2.01948638247731\\
-1.95716076840529	1.99607823761351\\
-0.0490020531298713	1.87166916789\\
-0.968221253441032	1.0371103158866\\
1.96655102998387	1.02516094716958\\
1.10271894975034	0.958503290863836\\
-0.953798190106776	2.04611125549924\\
0.0651790518884468	2.04563010105022\\
1.97001159480017	2.01815222399546\\
-2.02787311804674	1.95337025685468\\
1.04018080254003	1.82628607335721\\
0.925768361660823	1.09943182947283\\
-1.02904786375528	1.01472756895205\\
1.98708689064935	0.97190996478791\\
0.0628445106226954	2.06685567747021\\
1.93892844814504	2.06286190236403\\
-2.04145523757816	2.00365128558299\\
-0.97545427603597	1.95651503284232\\
1.07120413723658	1.8328429695065\\
0.971163951401785	1.08563347965794\\
-1.00508352989475	1.00526611943264\\
1.98323098701958	0.979130517019016\\
-1.97387536372941	2.11188877763797\\
2.04363188464564	2.02597038884017\\
0.032579342661976	1.9824911988984\\
0.891648005765711	1.93359285083424\\
-1.033869140237	1.90826655014623\\
1.03981653482957	1.04017830276205\\
-1.01559697564067	1.00369193867348\\
2.00603807088553	1.00044395370078\\
0.190233006946526	2.11425420482211\\
2.03883015687196	1.96773185816805\\
-0.986874549926133	1.95509298544894\\
-2.08906107998457	1.87026914612897\\
0.891609822702622	1.74564358160279\\
0.956180184778506	1.12209847830033\\
2.00364249290765	0.99269318404895\\
-1.00141999135928	0.961487417794718\\
-0.913978895753233	2.12790185685618\\
2.06371929850691	2.03681623282423\\
-2.05319014623152	1.9871043764663\\
-0.0635645734614863	1.9567826787231\\
1.00662585807425	1.78746882106088\\
1.00044437566249	1.09060828773674\\
1.98281769779837	1.01600661448493\\
-1.02126396721249	1.00316439758758\\
0.44165709678793	2.30153824000401\\
-1.95505836636727	2.00148248354344\\
2.02361534699977	1.96981395040194\\
-1.16649521858406	1.9436911659681\\
0.735167402028515	1.81596733761353\\
0.926856307875894	1.05750193274249\\
2.01520408230084	0.991450468340334\\
-0.970862713278239	0.950698800992715\\
1.04029184669499	2.06873924865602\\
-0.934943116250507	2.02936243774388\\
1.98571519378746	2.01245216323336\\
-2.01989949136813	1.99922365515956\\
-0.0830206965847511	1.90394312180814\\
2.00386445127102	1.01835619083479\\
-1.01326781783915	0.983033034188717\\
1.07791429766859	0.979919272524113\\
0.753900352554764	2.123316546968\\
-1.08284955936002	2.03738226658232\\
2.07229870709197	2.01485355830472\\
-2.02667228004269	1.98015565601871\\
0.184862943829805	1.75397371728522\\
-0.980450816938469	1.03597064878152\\
1.09832096309285	1.01446841014953\\
1.9892067520246	1.00431386133607\\
};
\addplot [color=mycolor2,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.994496712429657	2.13261600053448\\
-1.9388318589387	2.06779124425686\\
-1.04484515117617	2.03422465348894\\
0.0350351022709005	1.97179201854427\\
1.94087231829291	1.97106943650923\\
-1.03172933616519	0.998247365809088\\
0.983582007503909	0.99514941059542\\
2.03755929889099	0.978795794214106\\
1.06766947240552	2.06606644041898\\
1.96385515307763	2.0276588103648\\
-2.02048872038634	1.99209496378355\\
0.110557651240304	1.95701336133004\\
-1.03700271917097	1.91565440805652\\
1.01222720106275	1.03235594098236\\
2.00300024484782	0.992621082801248\\
-0.967924374694894	0.910463352156827\\
2.00620885651723	2.01414815959358\\
-0.012151490338812	1.99644092017344\\
-0.995119834421725	1.99634220442249\\
-2.02361054307812	1.97501443317535\\
1.0250712432571	1.96751490814321\\
-0.991393932019203	1.0146885505119\\
1.98393744466306	0.997503274386299\\
0.99013009479715	0.977540480434959\\
2.00521250489992	2.03582031103462\\
-1.0038784798329	2.02562055577385\\
-2.02880942288219	1.99630073978637\\
-0.0034547947839823	1.96846093951776\\
1.04623089069885	1.96617905404067\\
2.01257760547897	1.0357601728711\\
1.02432793996866	1.00694872142832\\
-0.991300788442007	0.993320347964434\\
-0.996476445857843	2.0404776506993\\
-2.02416626537862	2.02693853537112\\
2.00093170471043	2.00246733815394\\
-0.0637049754541589	1.95822962932325\\
0.996347595099872	1.90001316653159\\
1.01066719695706	1.09663643013234\\
-1.01094432560786	0.999019711385637\\
1.99835276119263	0.961659350431988\\
-1.00873756985429	2.04204872280879\\
-2.04916283125477	2.00130646621626\\
1.01010894860698	1.98424138122248\\
1.98367854028113	1.97073366686347\\
-0.0239767532227252	1.96031924445887\\
1.00404813048457	1.04906614388001\\
-0.999921796896312	1.02681566670236\\
2.00360556277416	0.981395481439347\\
0.884812137642156	2.07563834443956\\
0.0564363447250798	2.07233329491975\\
-1.98151552149363	2.03425048128996\\
-1.00507446972579	1.97876701110779\\
1.98061947152056	1.92855409315932\\
0.989344912751836	1.03897257632638\\
2.04218837794329	0.986833697448694\\
-0.943481513500937	0.967605963808284\\
-2.03457355327684	2.01122906375741\\
2.02030862546708	1.99758962518096\\
0.0491545547683462	1.99543554224651\\
1.03759336497349	1.9762306202794\\
-1.04176717215367	1.95379787121166\\
0.952405547557491	1.03997850062585\\
1.95743152449501	1.01166357165664\\
-0.929861066622552	0.998813198958324\\
-2.01585528279514	2.00329293187571\\
2.04245733484459	1.99989494438469\\
0.00333439002092505	1.99541482897923\\
-1.00470415796318	1.95384910744307\\
0.985447521814545	1.9365547750587\\
1.02565165403403	0.996444642244651\\
2.00949843750824	0.996124846385653\\
-0.995854395127349	0.979106922444181\\
0.998045299268938	2.02248774112544\\
0.0345736199384624	2.01725784810599\\
1.98715419129694	1.9931911330767\\
-0.975498446861587	1.95637917464506\\
-2.03898679697902	1.93206058835016\\
-1.00444375743331	1.01218419402978\\
1.00554085497534	1.00873358141696\\
2.02309481817987	0.99478448345983\\
0.0231371241194496	2.01587136923509\\
-2.04838557750681	2.00014042211582\\
1.01684259764907	1.99507730343694\\
1.99872942013274	1.99292806690254\\
-0.983259875227103	1.95052288074279\\
2.00953234594051	0.996055170850054\\
1.03467415462732	0.984786118838074\\
-1.02304430960412	0.972915806700797\\
-1.01615970837602	2.03536551507985\\
-0.0181099398427944	2.00181830217011\\
-1.97838939415994	1.99408905531308\\
1.96485034656478	1.98734355572473\\
0.981425603620803	1.94942952663438\\
1.0777140011099	1.07225208285461\\
1.96740386653254	1.01076592055345\\
-0.959128673326751	1.01042792480641\\
2.01770734472706	2.05017221621873\\
-0.951175379180508	2.0206910982516\\
-0.0817853000571831	2.00203813531839\\
-1.99824029966743	1.95116442759588\\
0.988595450662355	1.88952567379698\\
1.06634595602907	1.03929472874502\\
1.9436263382416	1.018381035713\\
-0.984501827326427	0.990880431162794\\
1.97577018833367	2.03111945477713\\
0.0280340403021818	1.98899344780783\\
-2.0713302954722	1.97146444537405\\
1.05014962195851	1.95286071797687\\
-1.00670455801632	1.91547858296028\\
1.01191963674509	1.04111556651398\\
-1.00990564199468	0.978083603969244\\
1.96866638821355	0.965039878846777\\
2.00281516870533	2.00092636896625\\
-0.979065319883836	1.99900587375234\\
-0.0305116376675263	1.98611608968672\\
-2.01487878430471	1.98364814148786\\
1.02517260666923	1.95132595448933\\
0.984768234045453	1.02699343819221\\
-1.03029816439895	0.993438175818983\\
1.97359302635945	0.974529462879405\\
2.00669220041569	2.01991634198462\\
-2.04520131492964	1.98688670347421\\
-0.999453651749145	1.98380460945689\\
0.0279597311195186	1.98209615217127\\
1.03253039248487	1.98157035972626\\
0.958960254997433	1.05137767441949\\
1.99015441031751	0.995498545621815\\
-0.957634205296289	0.985364146996903\\
-0.974076213965311	2.04158313084348\\
-0.0772207897833821	2.02924927447026\\
2.05083883506268	2.01296653533288\\
-1.9753370436407	1.97906123703181\\
0.918702296827976	1.91976118124965\\
1.05000079505506	1.04126360009197\\
1.94771570188202	1.01391088489721\\
-0.97195367981103	0.983850743183458\\
-0.00254655927159431	2.01180947174181\\
-0.997690770115005	1.97599656780931\\
0.950296211134705	1.96389405534586\\
-1.9826883682913	1.96346645024035\\
2.01224726248757	1.95702493941709\\
1.04075236985118	1.02749936217495\\
2.04123309549121	0.982994267543199\\
-1.03992052508126	0.965963386280785\\
-2.05339895138733	2.0244039389408\\
-1.05413624565366	2.01065602526866\\
0.974772376673797	1.99399870957575\\
1.98342466822184	1.97498568925716\\
0.012964117755839	1.96957908840496\\
-0.964801483619405	1.01787424301853\\
0.982212492775665	1.01296510912876\\
2.02166296967934	0.966785625182277\\
0.933632540976114	2.02514422150691\\
0.070793246231623	2.01589908122435\\
-1.99355910105677	1.99455972406835\\
2.01327490170085	1.98557664586022\\
-1.03082199603649	1.93660976793328\\
2.06983869729536	1.06485106058474\\
1.07313476873506	0.985209028202193\\
-0.984852724025589	0.954109150786403\\
1.04831859471812	2.06530972626289\\
-1.0549267204184	2.02204742783396\\
1.95588439410151	2.01251147818336\\
-1.95997024854917	2.00229340140179\\
0.0453948500293355	1.95301412858242\\
-0.990236269382984	0.984777742655168\\
1.99092216839263	0.976813505004939\\
0.998210158279353	0.976350396417539\\
-1.01398620410135	2.00737322257743\\
-2.04694731559452	1.98687328773056\\
1.98998624501413	1.98412121364219\\
0.0122864926034897	1.96235022241044\\
1.05989337861865	1.96164360085016\\
0.946327405028999	1.04379992412625\\
-1.00255086946638	1.00317173484264\\
2.00062505736042	0.983867043470906\\
-0.0187671898765218	2.06320633430332\\
-1.99983485885658	2.00740473238302\\
-1.0011130360985	1.98289486173809\\
2.02320005441713	1.97644108456998\\
0.929361193624029	1.93041469350354\\
2.01173787475321	1.00219166029207\\
-0.96059340125131	1.00104347055501\\
1.02773472757071	0.968770490285892\\
-2.02241781681538	2.01414940001906\\
0.00153974913656686	1.98412342618934\\
-1.02842846253539	1.98389123615912\\
0.94528798132113	1.97782851136135\\
2.02136715003402	1.95572075002411\\
1.03517603826822	1.01129282795322\\
-1.00917527655821	0.982209682497384\\
2.02194350477512	0.979641977191183\\
-0.043080908121251	2.05090571389574\\
-2.00013837043668	2.02863736072411\\
-1.01181108197435	1.98375368831178\\
2.04252696612342	1.95711057724075\\
0.910324724201138	1.92687294969824\\
2.0410790677787	1.01873465209375\\
-0.998517619608759	0.99477796454307\\
1.02974310645887	0.975157709236531\\
1.08239546426055	2.06559950021093\\
-1.04184538190329	2.03741573110494\\
-1.99280844388273	2.0328313191302\\
1.96448334908492	1.98689586449791\\
0.0366252626540283	1.98151248004654\\
-0.952867921823043	1.04528541751134\\
1.98638646497986	0.994611595326142\\
0.913682595350808	0.95092387325603\\
-1.03888041949979	2.06068548478039\\
-1.96917341733152	2.02833031094951\\
2.0152566650333	2.01487046509986\\
1.07323146116451	1.97005483854361\\
-0.0240460829460748	1.93577373594752\\
-1.0259118568997	1.01170674133095\\
0.944938927114206	0.995110600623936\\
1.98531302299764	0.988478164961428\\
0.986050779218429	2.06587263140385\\
-1.00540733819758	2.01814728622778\\
1.98853936832373	1.99812122024755\\
-2.01393751934277	1.99513208410464\\
0.0173104262696433	1.98598490599772\\
-1.02271805358594	1.0199853686307\\
2.01786312843393	1.00124495000387\\
1.03404487232567	0.963252444461542\\
-0.98359654857405	2.00561205643345\\
-2.02847106728641	1.99754329208397\\
2.04181857360658	1.99113206493823\\
-0.0443131782150867	1.98698588788245\\
1.00248507177194	1.9850585318374\\
2.00110415444487	0.982047394103919\\
-1.01394679495419	0.974937031975707\\
0.997323206372363	0.926890689328402\\
1.96520288160485	2.09427411463331\\
-0.99165805306349	2.00907377912233\\
1.12480261040925	2.00376213509811\\
0.0325848433125921	1.95992229160384\\
-1.96051489160289	1.92271837523388\\
1.04131549836711	1.02408648091136\\
-1.03588118590172	0.997247696327301\\
1.93315430861874	0.973701212162371\\
1.00003524920809	2.09164448094998\\
-1.99662259932343	2.07547311221326\\
0.0651792602428149	2.03954305327133\\
1.97714812192818	1.99631160557607\\
-1.03803863192529	1.97730082760423\\
-0.980333134085858	1.01397313376693\\
1.96933950939814	1.00029602246373\\
0.969799711422264	0.982809035659704\\
0.000396531920149969	2.08183252881904\\
0.931126728026833	2.00427289368367\\
2.00870257006166	1.99722123037606\\
-1.97136355335457	1.98897681844336\\
-0.975662510283235	1.95548282557961\\
2.00113900528077	1.01743715362309\\
-1.02846565503817	0.97042132273546\\
1.05234653651815	0.966640085260069\\
0.97802414250492	2.04050592161097\\
-2.00582334072607	2.00337061317635\\
-0.993990829460043	2.00085300672573\\
0.0162786887355209	1.99933231994254\\
1.98149637049207	1.96629932843224\\
0.96524538315017	1.018098660034\\
-1.00828061967117	0.993316205642106\\
2.00996122446138	0.947661686204233\\
1.00672596100231	2.05050601286711\\
0.059075907790443	2.02491527218387\\
1.97652292139071	1.99665123132111\\
-2.03287255556628	1.99045176707544\\
-0.992203642136795	1.97052966589543\\
0.986771372863226	0.983997768721697\\
2.01259425560112	0.983287093479521\\
-0.960622914261605	0.967980315949787\\
1.01251538911257	2.0707929855165\\
-1.98245838315212	2.01853967670842\\
-1.04092563355815	2.00273807706638\\
0.0359860153243598	1.99891195918877\\
1.99474949844926	1.97919647613964\\
-0.99948051399025	1.02276276462506\\
0.943272504700754	0.984656954720316\\
1.9655050196256	0.967297587098461\\
0.943861175317068	1.99579321887022\\
2.05064296617974	1.99158395804552\\
-2.02568426326198	1.98712986573271\\
0.0324867510493218	1.98443730389175\\
-1.02954534874356	1.97474703916297\\
2.0172775792563	1.03103179025231\\
-1.0052133153706	0.993299847211466\\
1.0566897156642	0.979498793851002\\
0.986898065601641	2.07598181279168\\
0.0926649187386036	2.01154870167627\\
1.97723673236686	2.00956928593222\\
-2.00410729013363	1.9949901705345\\
-1.02636052562085	1.95162554136415\\
1.99199873712559	1.02565361658348\\
1.03877761161357	1.00950042125857\\
-1.00032028799639	0.998488041416324\\
-1.97413424032168	2.00731178030304\\
0.96116684594924	2.0004462539181\\
-1.0135656810385	1.9997355812303\\
-0.00453470322019319	1.99542175445573\\
2.00271861644526	1.99461604638547\\
1.01937512421826	0.988167774362415\\
-1.01696170302739	0.980386717619997\\
2.02069089531618	0.972858975886658\\
-1.01596290572293	2.03815658571157\\
-1.96088342192331	1.99989020783921\\
-0.0442639010610087	1.99160290081839\\
2.02521765051006	1.98047872714544\\
0.977542303143686	1.9768113023204\\
2.01670079523058	1.0027978364515\\
-1.00897311777086	0.994908610496707\\
1.00547346736091	0.961932347016006\\
0.998238933480716	2.04254891992372\\
-0.996695577087756	1.99470802049593\\
-2.01471318299051	1.9929475406209\\
0.0210832082952795	1.97363606408353\\
1.99742958215175	1.97234785331287\\
0.987870056149238	0.997539237181782\\
-1.01946664236514	0.985477545199712\\
2.01965736424655	0.984290096425405\\
-1.97338859410988	2.04211235849341\\
-1.04255900181184	2.01636532441155\\
1.06482244611997	1.99553732715161\\
1.98455573575736	1.98863163254969\\
0.00340345185738475	1.9457096655378\\
2.00847100414944	0.997382067043549\\
0.968212616642068	0.991499492897423\\
-1.02172166258484	0.985222791974996\\
-1.0430654552374	2.01544080760522\\
-2.03850916603949	2.00376370214647\\
0.923826310781568	2.00285339015789\\
-0.0122383702479328	1.98635228923982\\
2.00177286183185	1.95366962295811\\
-1.00253017161222	1.09252684071472\\
0.991324104950812	0.995446876046817\\
2.02723745165749	0.96861017228308\\
0.999618314712776	2.00451058391565\\
1.96679816671134	1.98982077344812\\
-1.00538199200544	1.98660105088519\\
0.013902588044404	1.96712883765903\\
-1.99875165076149	1.9647565205348\\
1.03142770065207	0.999091228132049\\
2.02532464532217	0.946710761820171\\
-1.03642500946817	0.935636182070994\\
1.00322102066112	2.01430303479946\\
2.03577644640247	1.99295316117014\\
-1.99079049013736	1.98471140481103\\
-1.04485469104286	1.97839546289416\\
0.0321781059970663	1.97301072321076\\
2.00695016625705	1.0029111963445\\
-1.02540733164935	0.991915450489807\\
1.0096468969893	0.96758973044102\\
1.94605986259388	2.06345505805754\\
1.01087214754722	2.05137084899733\\
-2.01585794331444	2.03194816431457\\
0.0818593886943617	1.98663593753095\\
-1.05033415146643	1.96246048597683\\
1.04723477836738	1.05352372437251\\
1.99324982060487	1.0096093164188\\
-0.971498763242541	1.00459999847679\\
1.0530121987415	2.04485627340521\\
1.95330351155425	2.03506168782945\\
-1.0286666689254	2.0072478433359\\
-1.98038330686153	1.97635772054607\\
0.0456085999268988	1.95480338199233\\
1.04130812988161	1.01818709248869\\
1.99733644666498	0.995053113259349\\
-1.0000584757113	0.960358504734811\\
0.0366514480601331	2.02547855974686\\
-2.04319791191017	1.98289145840161\\
0.996839368624675	1.98102988640511\\
2.01109625585708	1.9675380911693\\
-0.979366609250543	1.93222228088565\\
1.01651399891906	1.01671392020568\\
2.03041826396976	1.01623009939118\\
-1.02807928962087	0.968931171383708\\
-2.01655582229422	2.02709936939948\\
1.99971122034069	1.99817936646025\\
0.00639654735011156	1.98535807604601\\
0.998024990450184	1.97224033692193\\
-1.01055188663862	1.95539665790057\\
2.02845880877947	0.987851811547164\\
1.06096077006404	0.978020078715756\\
-1.03367747086568	0.955271346768997\\
0.0166282821011586	2.02144800032971\\
-2.05127294615864	1.98539254984249\\
0.96523075662858	1.98452401933889\\
2.02583137930703	1.98107073818358\\
-1.00347586107154	1.95758267734608\\
1.99610598077493	1.03253962045557\\
1.04469065589308	1.02218020561515\\
-0.978743962225419	1.01663323035465\\
-2.00841513396218	2.01266307015881\\
0.0332872404043879	2.00356181104064\\
0.968544828909998	1.99173997461073\\
2.02797150987519	1.96474699877743\\
-1.04048314033692	1.95928922622829\\
-1.00841890095142	0.985660179742627\\
2.03402307985165	0.972727231090765\\
0.967754278203357	0.905097181858714\\
1.99294282750836	2.01595353979402\\
-1.99794462603102	2.00513583017856\\
-1.01800028438291	1.99388121283918\\
0.984665916707318	1.9729343143858\\
0.00955999085627313	1.97156609933467\\
2.04330847871135	1.00308963320792\\
1.04212634032602	0.985685716397553\\
-1.03589147894734	0.983245025922184\\
-2.02987079073119	2.04002681216413\\
2.00869452629965	2.0389218395289\\
1.00626522751839	2.00925275391777\\
0.0291063121762224	1.99135168792393\\
-1.04364618717987	1.95847441915925\\
1.99968542662065	1.0069172491236\\
-0.988480001206919	0.999353411576864\\
1.02104006546109	0.959598439183873\\
-2.00737901273801	2.02178887767775\\
-0.0410668230587008	1.99616676786831\\
1.0715910297983	1.99498881842885\\
-0.981547149847306	1.99380147086797\\
2.00294363562203	1.99044652315455\\
0.94602338697236	1.05105336029409\\
1.95054845417228	0.978386669533141\\
-0.997348346167229	0.975188071196511\\
-1.00033366028711	2.04496071126161\\
-0.0143131778830961	2.02114687071364\\
1.01980784973079	2.01531462506488\\
1.98037133003526	2.00742333539043\\
-2.06002803817732	1.98562620978045\\
-0.953311157576043	1.10525628588682\\
0.957319526071867	1.00689878175269\\
1.94683516005521	1.00053587156302\\
0.00390066717041661	2.00896606406644\\
-2.01520283447907	1.99519127210743\\
-1.02009007969315	1.9940370864086\\
0.992121331357042	1.99379933296874\\
2.02860587025271	1.96411334275194\\
-0.988110930419037	1.03099126191571\\
0.950186785862589	1.00594852730198\\
2.02006985970734	0.99729718840803\\
2.03192089828194	2.02739659036481\\
-1.00755352802758	2.01646921764888\\
-2.00934905398883	1.9739080325994\\
0.95889852023369	1.96726082350049\\
-0.0391734445555418	1.96137701102388\\
1.02085647096773	1.01615142059627\\
-1.01355551698481	0.998237309349675\\
1.98151652957221	0.942909257857198\\
-0.00246496965511841	2.08149019621864\\
-1.97682490552205	2.05846681776646\\
2.03392214363043	1.97706289318275\\
0.93815254196789	1.97296565910423\\
-1.00278973892581	1.95981283146089\\
0.99224939511422	1.03124951789286\\
1.97998084375517	1.0252209427014\\
-0.965966115627329	0.947441783912799\\
-2.01442241949618	2.03219485026382\\
-1.03583591385024	2.02458483038903\\
1.07822096458301	2.01361917329693\\
1.97762892116662	2.01051587466879\\
0.00287849747718266	1.94742206485364\\
-1.02257141840125	1.01981281551655\\
1.99461720407923	0.971802488754083\\
0.964052927985042	0.971350126521171\\
1.01253175984464	2.0417606596739\\
0.0505285866947772	2.01235819962007\\
2.0107181948459	2.00972486301239\\
-2.0068952133862	1.98058936646249\\
-1.00976376979108	1.96744336849377\\
1.97474188671853	1.01967580844412\\
-0.981850866612273	1.0034489475747\\
0.996008556127393	0.974011798741872\\
1.02241269955129	2.00325812870258\\
2.02517256152789	1.98648954015796\\
-1.0101178484618	1.98401820383862\\
0.0435223195649752	1.95813289201874\\
-2.0393545274722	1.94548343858271\\
-1.02515150013394	1.05159285005609\\
2.02753242818793	0.993837664476325\\
1.01056191358015	0.978872490643072\\
1.02932405353795	2.02277224353046\\
0.030528428239941	2.0226351184538\\
1.98678000556029	2.01712915192906\\
-2.02947189581176	1.97239673447415\\
-0.980851505497382	1.95827489035895\\
-0.975078511661037	1.00586867941127\\
1.97685147783414	1.00079932712818\\
0.996199745024038	0.987188995275188\\
0.0601494119624386	2.04392285544179\\
0.972264721249343	2.0128976696492\\
-2.03413666200833	1.99792697276481\\
2.00514468068735	1.98235688409352\\
-1.0098619530414	1.935573976918\\
-0.982344216984797	0.99904595297231\\
2.00092664750145	0.982786972033498\\
0.960610118868105	0.951585501703255\\
-2.04702613997156	2.02364642900718\\
-1.01993866439611	1.98141586862879\\
1.9988744604951	1.97157243294935\\
-0.00622909634472796	1.93631876244417\\
0.994458094931841	1.93148579530073\\
1.10131421191161	1.05584900307317\\
2.0355595239689	1.01487338146283\\
-1.03713165081591	0.982306513420515\\
0.962215817880924	2.01653614081539\\
-2.01766475756369	2.01380533045088\\
-1.0170443181929	2.00467310677512\\
-0.0103051767774415	1.99670521411504\\
2.02351997807369	1.94758852684126\\
-1.02131164541122	1.0139616419116\\
2.02286364105295	0.958004524760291\\
0.989371780564868	0.954451472313281\\
-2.0101789537969	2.03261616125209\\
-1.01619746265442	1.98945523847628\\
-0.0385410583471691	1.9816451228445\\
0.954101748846274	1.97180633731544\\
2.02153706817998	1.97032350525946\\
1.05360731090082	1.00902715178987\\
2.0414467369566	0.993936350997468\\
-1.03069129078959	0.948880273130058\\
0.018609573473527	2.01618158771565\\
-2.01342314593571	2.00644559498948\\
2.02473647401037	2.00371064959187\\
-1.00549418271742	1.95866810674897\\
0.968461907935807	1.94636987138303\\
2.00746940131014	1.01028477836938\\
1.0326106127816	1.00921644404082\\
-0.961825148410457	0.96334964895521\\
0.938766183232256	2.01189684782407\\
-1.00182397169576	2.01121480774323\\
-0.00949665434027599	1.99565695155148\\
-1.99814574804188	1.98883577004611\\
1.99838142926012	1.94566675908954\\
-0.999055645406724	1.0196633341108\\
1.02151448266246	1.00320375982526\\
2.02598930355202	0.974486449691552\\
-1.00353289544965	2.013276942124\\
0.964081300237453	2.00560146097477\\
-0.00642860463614912	2.00038915616627\\
-1.98131363128412	1.97937320272055\\
2.00032305018194	1.96763861341601\\
-1.01373702060745	1.02047271674818\\
2.03623880934698	0.991230645386857\\
1.00981706717377	0.948515430137893\\
-1.97939579415199	2.03083164537621\\
-1.03865675548831	2.02055251774752\\
2.00191667091773	2.00987151983382\\
0.968596903076147	1.97009583187216\\
-0.023456912135443	1.96568044964234\\
1.0088408308954	1.0002938587025\\
-1.0051179307906	0.982279690484461\\
2.01094055047948	0.957886411765789\\
-0.998161228151219	2.04177918265066\\
2.00806030674885	2.00456854422932\\
0.995066617227318	1.99576770550751\\
-1.99244402920321	1.98551650028612\\
-0.0233925293507033	1.9697725590533\\
0.997947144844541	1.01542456136587\\
-1.01455730936653	1.01309664281077\\
1.99279720295135	0.966507545611842\\
-1.9531142043929	2.06070722580005\\
-0.0143243014303224	1.99189048407067\\
0.936759803583676	1.99034486879721\\
2.03288362461206	1.98780803166375\\
-1.04309662153058	1.98761214984844\\
1.04155557325355	1.00856545238626\\
2.0035831905219	1.00285109665817\\
-0.997948872596773	0.954836055691048\\
-0.984028096471111	2.07409259178037\\
2.02463345040516	2.0294672901489\\
-0.0338989311787165	1.9823552140585\\
0.979615391365537	1.97078373098851\\
-1.93944223492955	1.96443387569893\\
-1.03796190385041	1.01682539796821\\
2.01766028067548	0.99194697864228\\
1.01037164670728	0.937010525221403\\
-2.01394625097455	1.99454641200482\\
0.984151426949383	1.98240542065717\\
0.00660940874750213	1.97470936975686\\
-1.03262534278619	1.9738929595002\\
2.01992793149493	1.96720984645462\\
-1.03718550321424	0.992804872648921\\
0.999348898325653	0.9770483781932\\
2.02513119344869	0.974008828288252\\
-1.98446617156839	2.04742791425972\\
-1.02606032011108	2.00428075493402\\
1.97878572645997	1.98439193811131\\
0.993819155079608	1.97814601160874\\
0.00438527035712546	1.974769404134\\
1.00666048167422	1.00608392159397\\
-1.00324463568201	0.998871510824483\\
2.03072857209953	0.973544696655724\\
0.00414653579536946	2.04107467030883\\
2.02151196814385	2.0001895876807\\
-1.99538272542307	1.973627097412\\
-0.999079409982093	1.97196505720453\\
0.952707739088452	1.94901919454695\\
2.01176739433912	1.03978255812111\\
-0.984447404723992	0.996771282949005\\
1.05421214935082	0.960274395706415\\
1.02585608920746	2.07682412824123\\
-2.02316534034677	2.06918910880269\\
1.96857550488277	1.96707078487938\\
-1.05559228308407	1.9658684124596\\
0.0495934015999718	1.96111105763038\\
0.973664786872513	0.978214482453529\\
-0.97366910329772	0.972789880682026\\
2.01100322627089	0.969112185653527\\
-1.99816686536282	2.02177600356601\\
0.0464111697045952	2.01532601109898\\
1.00180142917916	2.00684869859123\\
2.00051272901867	1.97562022241716\\
-0.996713470872247	1.96444211280605\\
0.993660113498255	1.0287338999951\\
2.0033373279761	1.0232429182672\\
-0.993108193052089	0.944573806316699\\
1.99703508576355	2.07375394430503\\
-0.0683316097564047	2.03991200856391\\
-0.892891576454235	2.02302397691021\\
1.09135067045937	1.91965331842093\\
-1.981270453505	1.91812152372371\\
0.997945085101291	1.11395359811383\\
-1.04093659306311	1.03993905292803\\
1.91143399029914	1.02054409341476\\
0.993037064759998	2.01320790880762\\
0.0467376982868822	1.99964135017553\\
2.03518953383324	1.9956258069959\\
-0.997059959102544	1.95708302796415\\
-1.99785268087751	1.93975022595144\\
2.02790590322098	0.998343894528205\\
-1.05614150327378	0.960915844033726\\
1.02419931150803	0.95668918507693\\
2.0040882666162	2.05357148904045\\
-0.979081327292665	2.00771311649935\\
-2.04430865385224	1.94133948886097\\
1.02890684381565	1.9329358067054\\
-0.0197132093318205	1.92865513355101\\
1.04748580184934	1.04242491667413\\
2.01414726576863	0.995900411514671\\
-1.03019435323456	0.977362753934826\\
-0.0244888139061857	2.09055125805133\\
2.02238794871983	2.02336517588728\\
-1.99035877897016	2.00157886679821\\
0.993971109345445	1.98544318610679\\
-0.947172468334514	1.9574210963389\\
1.976504544696	1.02354844030679\\
1.0318612644531	0.986773592747212\\
-1.01091064167652	0.97196989630449\\
1.02192279190529	2.05363974701636\\
1.98507270705688	2.01391903443682\\
-1.07675734993571	2.01349369693584\\
-1.9684838805378	1.99882204830819\\
0.055134342479738	1.93024715557554\\
2.02674671341256	0.990256751139595\\
-1.01564387420762	0.987703540732723\\
1.00104355015525	0.964251679854576\\
0.0237856028299167	2.04651815808515\\
0.948255947087048	2.01489161571538\\
1.97309251651855	1.97663020113386\\
-0.975455126555253	1.97450327628475\\
-2.0282620509476	1.963551354837\\
-0.998878820397639	1.04288156892224\\
1.02820163272564	0.970975933909699\\
1.99003756928481	0.970577865296297\\
-0.00210940374476524	2.02771956229467\\
2.0006013025625	2.01211998807885\\
-2.02153102728893	2.00217562519857\\
0.950984887857542	2.00088829009708\\
-0.999049755418776	1.9756457207027\\
1.99693711470128	1.01205907319354\\
1.06399546952397	0.990331884133461\\
-1.00035233680372	0.979116416741888\\
1.0218597743356	2.06888654026157\\
-1.96422311358405	2.032624781553\\
-1.07179252289759	2.00724527830426\\
1.92113584432633	1.96656028390426\\
0.0612073690909163	1.94020141950343\\
0.998003155754578	1.0354098592665\\
2.05494769540495	0.972353394038427\\
-1.00509459422724	0.968798045161362\\
-0.040980795833023	2.03432571554143\\
-0.973104164218677	2.01739605249412\\
2.01145178218246	2.00586997714905\\
-1.9898943215972	1.99681923000407\\
0.9349142819555	1.97867997179208\\
1.99676535635601	1.01423249589344\\
1.06240240507625	0.999269258526421\\
-0.976738574426631	0.944560410623854\\
2.00376467180919	2.07332004487268\\
-1.02534852999695	1.99710910066684\\
1.08689078999724	1.96894226777464\\
-1.97346370764085	1.9644489420022\\
0.0332687745642912	1.96034878734134\\
-0.986870752651638	1.00844977707271\\
0.993835549692264	1.00784185112008\\
1.95772348120802	0.977456365854185\\
1.99669345093629	2.03710356936964\\
1.02876664465916	1.98006890557238\\
-1.0069894799088	1.97720968749272\\
0.0320760702360778	1.97536195582432\\
-2.01925870686434	1.94683095359064\\
-1.00109945779973	1.01435734374926\\
1.99483598390736	1.00851135389617\\
1.03833637732533	1.00026352116567\\
1.99807575737868	2.00655095217728\\
1.0208306869195	1.99568728893843\\
-1.01395156390321	1.98807288804871\\
0.0161357400908766	1.97438970983644\\
-2.00581250831845	1.96503337233019\\
-1.04471608438893	1.01690731438995\\
2.00395122382182	0.983755614156768\\
1.01107481132809	0.943195561860214\\
-1.01567983555006	2.04746415955853\\
2.02031812367373	2.02235007762245\\
-1.9939116358024	1.9919151801013\\
-0.0472078901306351	1.96371996244096\\
1.00775757050882	1.91456628422766\\
-1.03132825424558	1.03115339735372\\
1.99552729154095	1.02191942255413\\
1.03880021721129	1.01250928281366\\
-2.06323562638865	1.97868993100256\\
2.02879407959929	1.97381185393215\\
-1.0193109449957	1.97201107926338\\
0.00535725367453169	1.95334678175664\\
1.03503582741868	1.91390610310938\\
-0.96904842019307	1.03631327676242\\
0.993339846373201	1.02952754988446\\
1.97654188697231	1.00832463349878\\
-2.01414545301726	2.02381196557783\\
2.00551270224116	2.00742160221399\\
-1.04208644965979	1.97976109647028\\
0.00599049563108294	1.95206184216546\\
1.06731375734407	1.92774417639828\\
0.982758446807234	1.07047441072373\\
1.97544149314947	0.999338323893843\\
-0.981666720018074	0.978224923485078\\
0.990134733281253	2.0255712573646\\
-1.01878881788916	2.0005640982362\\
2.02164055974681	1.98906113265213\\
-2.00503078293902	1.98410559310386\\
0.0186049267964393	1.98388391667732\\
-1.01676933753954	1.00100647538833\\
2.02178429797445	0.993297858282772\\
0.975238758291842	0.947718665317765\\
-1.97994881769084	2.04461810891835\\
2.00350568009553	2.02830743605605\\
-1.02141473490563	2.01502184463227\\
0.000305085980677401	1.99838899142254\\
1.02114111555404	1.98618895348282\\
1.98173688480997	1.03365802857307\\
-0.971519913401958	1.0121180650424\\
0.990093433806004	0.979348500285853\\
1.00816841810728	2.05597657752965\\
-1.02413480978156	1.99768180905821\\
-1.97847246172994	1.9923891703629\\
0.0638245484176834	1.98631026195342\\
1.94897290972701	1.98065332514664\\
1.02693212924149	1.0346968651516\\
2.0130259161746	0.962424588323654\\
-0.979132481410507	0.910409948032782\\
0.0346294472782901	2.03703090770928\\
-2.04651880647493	1.99907909610087\\
1.99123535855108	1.99258370182268\\
0.996542168752784	1.98693617122103\\
-0.998861755386488	1.96022226186301\\
1.98780405378907	1.02100503889549\\
1.01745775523623	1.00355762439862\\
-0.982067216789203	1.00081746461342\\
-1.0860146273446	2.01000954012003\\
2.01710554295639	2.00482408919229\\
1.04546834163926	1.99939694893023\\
-1.99992386207319	1.97833612275892\\
0.0324989811611135	1.91215064311231\\
-1.00293962139561	1.03935413676975\\
1.99354396956595	1.02141214181712\\
1.00412607752629	0.972537093076047\\
-2.01183377849588	2.0040733796614\\
-1.01440755243036	1.98536398482095\\
-0.0299373046559238	1.97850696225074\\
2.02561834260989	1.9627169888358\\
1.00375934871239	1.93645359227808\\
1.00212647612751	1.00861145226718\\
1.98206790993929	0.980910933393758\\
-1.00714117102423	0.953361381343943\\
1.05553061160183	2.02494923950228\\
2.00672852924856	2.01912405203325\\
-1.99330568030307	2.00332224489558\\
0.0433925464393693	1.99079179001763\\
-1.01124983437714	1.94956991280763\\
1.00050026845584	1.01177366974288\\
1.97903589611711	0.996436757309316\\
-1.00609163368154	0.951675342551184\\
-1.03887713421148	2.01584343922414\\
2.01104302696464	2.01557376540149\\
-2.03434617084186	1.97411618889333\\
1.04912437969348	1.97406594213519\\
-0.00814914210613179	1.96709634726984\\
-0.972478716433623	1.04433155422498\\
1.97249483308798	0.994950281309415\\
0.953739458567534	0.979166878168185\\
};
\addplot [color=black,line width=3.0pt,mark size=4.0pt,only marks,mark=x,mark options={solid},forget plot]
  table[row sep=crcr]{%
0	1\\
};
\addplot [color=black,line width=3.0pt,mark size=4.0pt,only marks,mark=x,mark options={solid},forget plot]
  table[row sep=crcr]{%
-2	1\\
};
\end{axis}%
%\end{tikzpicture}%
